A New Analysis of Differential Privacy's Generalization Guarantees

We give a new proof of the "transfer theorem" underlying adaptive data analysis: that any mechanism for answering adaptively chosen statistical queries that is differentially private and sample-accurate is also accurate out-of-sample. Our new proof is elementary and gives structural insights that we expect will be useful elsewhere. We show: 1) that differential privacy ensures that the expectation of any query on the posterior distribution on datasets induced by the transcript of the interaction is close to its true value on the data distribution, and 2) sample accuracy on its own ensures that any query answer produced by the mechanism is close to its posterior expectation with high probability. This second claim follows from a thought experiment in which we imagine that the dataset is resampled from the posterior distribution after the mechanism has committed to its answers. The transfer theorem then follows by summing these two bounds, and in particular, avoids the "monitor argument" used to derive high probability bounds in prior work. An upshot of our new proof technique is that the concrete bounds we obtain are substantially better than the best previously known bounds, even though the improvements are in the constants, rather than the asymptotics (which are known to be tight). As we show, our new bounds outperform the naive "sample-splitting" baseline at dramatically smaller dataset sizes compared to the previous state of the art, bringing techniques from this literature closer to practicality.

==> linear_query.tex <==
%!TEX root = main.tex
\iffalse %removing the warmup from this file
\section{An Elementary Proof of the Transfer Theorem}
\subsection{Warmup: $(\epsilon,0)$-Pointwise Indistinguisability}
\label{sec:warmup}

The first step in our argument is to show that whenever a transcript is generated by a pointwise indistinguishable estimator, that no matter what the original data distribution was, the \emph{posterior} expectation of any query $q$ conditioned on the transcript is close to its prior (true) expectation.

\begin{lemma}
\label{lem:exp}
If $M$ is $(\epsilon,0)$-pointwise indistinguishable, then for any data distribution $\cP$ and any linear query $q$, if $S \sim \cP^n$, with probability 1 over the draw of $\pi \sim \textrm{Interact}(M, A; S)$:
$$\left|q(Q_\pi) - q(\cP)\right| \leq e^\epsilon - 1$$
%$$\left|\E_{S \sim Q_\pi}[\frac{1}{n}\sum_{i=1}^n q(S_i)] -  \E_{S \sim \cP^n}[\frac{1}{n}\sum_{i=1}^n q(S_i)]\right|  \leq \max(e^\epsilon -1, 1-e^{-\epsilon}) = e^\epsilon-1$$
\end{lemma}
This statement is driven by a simple observation that follows directly from the definition of pointwise indisinguishability:
\begin{lemma}
\label{lem:tech1}
If $M$ is $(\epsilon,0)$-pointwise indistinguishable, then for any data distribution $\cP$ and any linear query $q$, if $S \sim \cP^n$, with probability 1 over the draw of $\pi \sim \textrm{Interact}(M, A, f; S)$, for every $x \in \cX$ and $i \in [n]$:
$$e^{-\epsilon} \Pr[\pirv = \pi] \leq \Pr[\pirv = \pi | S_i = x] \leq e^\epsilon \Pr[\pirv = \pi]$$
\end{lemma}
\begin{proof}
We simply expand the definition:
\begin{eqnarray*}
\Pr[\pirv = \pi] &=& \sum_{\boldx_{-i}}\sum_{x_i}\Pr[S_{-i} = \boldx_{-i}]\cdot \Pr[S_i = x_i]\cdot \Pr[\pirv = \pi | S = (\boldx_{-i},x_i)] \\
&\leq& e^\epsilon \sum_{\boldx_{-i}}\sum_{x_i} \Pr[S_{-i} = \boldx_{-i}]\cdot \Pr[S_i = x_i]\cdot \Pr[\pirv = \pi | S = (\boldx_{-i},x)] \\
%&=&e^\epsilon \sum_{\boldx_{-i}}\Pr[S_{-i} = \boldx_{-i}]\cdot \Pr[\pirv = \pi | S = (\boldx_{-i},x)] \\
&=& e^\epsilon \Pr[\pirv = \pi | S_i = x]
\end{eqnarray*}
The reverse inequality follows symmetrically.
\end{proof}
The proof of Lemma \ref{lem:exp} now follows by an elementary calculation that expands the definitions and applies Bayes' rule:
\begin{proof}[Proof of Lemma \ref{lem:exp}]
\begin{eqnarray*}
q(Q_\pi) &=& \E_{S \sim Q_\pi}[\frac{1}{n}\sum_{i=1}^n q(S_i)] \\
&=& \frac{1}{n} \sum_{i=1}^n \E_{S \sim Q_\pi}[q(S_i)] \\
%&=& \frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \Pr_{S \sim Q_\pi}[S_i = x] \\
&=& \frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \Pr [S_i = x | \pirv = \pi] \\
&=&\frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \frac{\Pr [\pirv = \pi | S_i = x ] \cdot \Pr [S_i = x]}{\Pr[\pirv = \pi]} \\
&\leq&\frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \frac{e^\epsilon \Pr [\pirv = \pi] \cdot \Pr [S_i = x]}{\Pr[\pirv = \pi]} \\
&=& e^\epsilon \cdot \frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \Pr [S_i = x] \\
%&=& e^\epsilon \cdot \E_{S \sim \cP^n} [\frac{1}{n}\sum_{i=1}^n q(S_i)] \\
&=& e^\epsilon \cdot q(\cP)
\end{eqnarray*}
Here, the inequality follows from Lemma \ref{lem:tech1}. Symmetrically, we can show that: $q(Q_\pi) \geq e^{-\epsilon} q(\cP)$. Hence, we obtain:
$$ (e^{-\epsilon} - 1) \le (e^{-\epsilon} - 1) \cdot q(\cP) \le q(Q_\pi) -  q(\cP) \leq (e^\epsilon - 1) \cdot q(\cP) \leq (e^\epsilon-1)$$
\end{proof}

Next, we present the simple ``Bayesian Resampling Lemma'' that drives our thought experiment. It tells us that when analyzing the sample accuracy of our mechanisms, we can without loss of generality pretend that the dataset $S$ is \emph{resampled} from the posterior distribution on datasets conditioned on the transcript $\pi$, after $\pi$ has been realized.

\begin{lemma}[Bayesian Resampling Lemma]
\label{lem:resamp}
Let $E \subseteq \cX^n \times \pispace$ be any event. Then:
$$\Pr_{S \sim \cP^n, \pirv \sim I(S)}[(S, \pirv) \in E] = \Pr_{S \sim \cP^n, \pirv \sim I(S), S' \sim Q_{\pirv}}[(S', \pirv) \in E]$$
\end{lemma}
\begin{proof}
This follows from the expansion of the definition, and an application of Bayes Rule.
\begin{eqnarray*}
\Pr_{S \sim \cP^n, \pirv \sim I(S), S' \sim Q_{\pirv}}[(S', \pirv) \in E] &=& \sum_{\boldx}\sum_{\pi}\sum_{\boldx'} \Pr[S = \boldx ] \Pr[\pirv = \pi | S = \boldx] \Pr[S' = \boldx' | \pirv = \pi] \1 [(\boldx', \pi) \in E]\\
&=& \sum_{\pi}\sum_{\boldx'}\Pr[\pirv = \pi] \Pr[S' = \boldx' | \pirv = \pi] \1 [(\boldx', \pi) \in E]\\
&=& \sum_{\pi}\sum_{\boldx'}\Pr[\pirv = \pi] \Pr[S = \boldx' | \pirv = \pi] \1 [(\boldx', \pi) \in E]\\
&=& \sum_{\pi}\sum_{\boldx'} \Pr[\pirv = \pi] \frac{\Pr[\pirv = \pi | S = \boldx'] \cdot \Pr[S = \boldx']}{\Pr[\pirv = \pi]} \1 [(\boldx', \pi) \in E] \\
&=&\Pr_{S \sim \cP^n, \pirv \sim I(S)}[(S, \pirv) \in E]
\end{eqnarray*}
\end{proof}
%\sn{If you cancel the terms in the last line you just get what you started with, shouldn't the proof just be:}
%\sn{begin}
%\begin{eqnarray*}
%\Pr_{S \sim \cP^n, \pirv \sim I(S), S' \sim Q_{\pirv}}[(S', \pirv) \in E] &=& \sum_{\boldx}\sum_{\pi}\sum_{\boldx'} \Pr[S = \boldx ] \Pr[\pirv = \pi | S = \boldx] \Pr[S' = \boldx' | \pirv = \pi] \1 [(\boldx', \pi) \in E]\\
%&=& \sum_{\pi}\sum_{\boldx'}\Pr[\pirv = \pi] \Pr[S' = \boldx' | \pirv = \pi] \1 [(\boldx', \pi) \in E]\\
%&=&  \sum_{\pi}\sum_{\boldx'}\Pr[\pirv = \pi] \Pr[S = \boldx' | \pirv = \pi] \1 [(\boldx', \pi) \in E] \\
%&=&\Pr_{S \sim \cP^n, \pirv \sim I(S)}[(S, \pirv) \in E]
%\end{eqnarray*}

%Where the substitution $\Pr[S' = \boldx' | \pirv = \pi]  = \Pr[S = \boldx' | \pirv = \pi]$ follows by definition of $Q_{\pi}$.
%\sn{end}

Finally, we observe that a consequence of the Bayesian Resampling Lemma is that sample-accurate mechanisms must in fact be accurate with respect to the posterior distribution they induce.

\begin{lemma}
\label{lem:posterioraccuracy1}
Suppose that $M$ is $(\alpha,\beta)$-sample accurate with respect to $f$. Then for every $j$ indexing a linear query it also satisfies:
$$\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A,f;S)}[|a_j - q_j( Q_{\pirv})| \geq \alpha +\sqrt{\beta}] \leq \sqrt{\beta}$$
\end{lemma}
\begin{proof}
Fix an index $j$. By the guarantee of $(\alpha,\beta)$-sample accuracy and the Bayesian resampling Lemma \ref{lem:resamp},

\begin{eqnarray*}
\beta &\geq& \Pr_{S \sim \cP^n, \pirv \sim I(S)} [|q_j(S) - a_j| \geq \alpha] \\
 &=& \Pr_{S \sim \cP^n, \pirv \sim I(S), S' \sim Q_{\pirv}} [|q_j(S') - a_j| \geq \alpha] \\
\end{eqnarray*}
%For any realization $\pi$ of $\pirv$ (which determines $q_j,a_j$) and dataset $S'$,
Let $E(\pirv,S')$ be the event that $|q_j(S') - a_j| \geq \alpha$. We therefore have that:
$$\E_{S \sim \cP^n,\pirv \sim I(S)}[\Pr_{S' \sim Q_{\pirv}}[E(\pirv,S')]] = \Pr_{S \sim \cP^n,\pirv \sim I(S),S' \sim Q_{\pirv}}[E(\pirv,S')]
\leq \beta$$
By Markov's inequality:
$$\Pr_{S \sim \cP^n,\pirv \sim I(S)}[\Pr_{S' \sim Q_{\pirv}}[E(\pirv,S')] \geq \sqrt{\beta}] \leq \sqrt{\beta}$$
Let $G = \{\pi \in \pispace : \Pr_{S' \sim Q_{\pi}}[E(\pi,S')] \leq \sqrt{\beta}\}$ (so $\Pr[\pirv \in G] \geq 1-\sqrt{\beta}$). For any $\pi \in G$, we must have:
%$$(1-\sqrt{\beta})(a-\alpha)\leq \E_{S' \sim Q_{\pi}}[\frac{1}{n}\sum_{i=1}^n q_j(S'_i)] \leq (1-\sqrt{\beta})(a+\alpha) + \sqrt{\beta}$$
\begin{eqnarray*}
q_j (Q_\pi) &=& \E_{S' \sim Q_{\pi}}[q_j(S')] \\
&=& \underbrace{\E_{S' \sim Q_{\pi}}[q_j(S')|E(\pi,S')]}_{\le 1} \cdot \underbrace{\Pr_{S' \sim Q_{\pi}} [E(\pi,S')]}_{\le \sqrt{\beta}} + \underbrace{\E_{S' \sim Q_{\pi}}[q_j(S')|\neg E(\pi,S')]}_{\le a_j + \alpha} \cdot \underbrace{\Pr_{S' \sim Q_{\pi}} [\neg E(\pi,S')]}_{\le 1} \\
&\leq& a_j + \alpha + \sqrt{\beta}
\end{eqnarray*}
Similarly:
\begin{eqnarray*}
q_j (Q_\pi) &=& \E_{S' \sim Q_{\pi}}[q_j(S')] \\
&\geq& \underbrace{\E_{S' \sim Q_{\pi}}[q_j(S')|\neg E(\pi,S')]}_{\ge a_j - \alpha} \cdot \underbrace{\Pr_{S' \sim Q_{\pi}} [\neg E(\pi,S')]}_{\ge 1-\sqrt{\beta}} \\
&\ge& (a_j-\alpha)(1-\sqrt{\beta}) \\
&\geq& a_j-\alpha -\sqrt{\beta}
\end{eqnarray*}
We therefore have that for $\pi \in G$,
$$
| q_j (Q_\pi) - a_j | \le \alpha + \sqrt{\beta}
$$
Since $\Pr[\pirv \in G] \geq 1-\sqrt{\beta}$, this proves the claim.
\end{proof}

Finally, we can put together the pieces to prove the transfer theorem:

\begin{theorem}[Transfer Theorem for $(\epsilon,0)$-Pointwise Indistinguishablity]
\label{thm:transfer1}
Suppose that $M$ is $(\epsilon,0)$-pointwise indistinguishable and $(\alpha,\beta)$-sample accurate with respect to $f$. Then for every $j$ indexing a linear query it also satisfies:
$$\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A,f;S)}[|a_j - q_j(\cP)| \geq \alpha +\sqrt{\beta}+(e^\epsilon-1)] \leq \sqrt{\beta}$$
i.e. it is $(\alpha', \sqrt{\beta})$-distributionally accurate with respect to $f$ for $\alpha' = \alpha +\sqrt{\beta}+(e^\epsilon-1)$.
\end{theorem}
\begin{proof}
By the triangle inequality, for any $j$:
$$|a_j - q_j(\cP)| \leq |a_j - q_j( Q_{\pirv})| + |q_j( Q_{\pirv}) - q_j(\cP)|.$$
Lemma \ref{lem:exp} bounds the 2nd term: with probability 1 over the choice of $\pi$, $|q_j( Q_{\pirv}) - q_j(\cP)| \leq e^\epsilon-1$. Lemma \ref{lem:posterioraccuracy1} bounds the first term: with probability $1-\sqrt{\beta}$ over the choice of $\pi$, $|a_j - q_j( Q_{\pirv})| \leq \alpha + \sqrt{\beta}$.
\end{proof}

Finally, we use an argument from \citet{BNSSSU16} to lift our guarantee of distributional accuracy to a guarantee of uniform distributional accuracy\footnote{This is sometimes referred to as a \emph{monitor} argument, but we don't use that terminology here because it is distinct from the monitor argument that \citet{BNSSSU16} use to obtain high probability bounds, which is the technique that we manage to avoid via our alternative proof.}.
\sn{a bit confused where we are using \cite{BNSSSU16}, if its to show that the below properties hold for our choice of $f_{lift}$ then we should make that a little more explicit. More generally, this falls out immediately from post-processing right?}
\begin{lemma}[\cite{BNSSSU16}]
\label{lem:monitor}
Suppose that $M$ is $(\alpha,\beta)$-uniformly sample accurate. There exists a post-processing function $f_{\textrm{lift}}:\pispace\rightarrow\pispace$ such that:
\begin{enumerate}
\item $M$ is $(\alpha,\beta)$ sample accurate with respect to $f_{\textrm{lift}}$, and
\item If $M$ is $(\alpha',\beta')$-distributionally accurate with respect to $f_{\textrm{lift}}$, then $M$ is $(\alpha',\beta')$-uniformly distributionally accurate.
\end{enumerate}
\end{lemma}
\begin{proof}
Write $\pi = ((q_1,a_1),\ldots,(q_k,a_k))$. Take $f_{\textrm{lift}}(\pi) = ((q_{j^*},a_{j^*}))$, where $j^* = \arg\max_j |a_j - q_j(\cP)|$. The two properties follow immediately:
\begin{enumerate}
\item $|a_{j^*} - q_{j^*}(S)| \leq \max_j |a_{j} - q_{j}(S)| \leq \alpha$ with probability $1-\beta$, and
\item $\max_j |a_j - q_j(\cP)| = |a_{j^*} - q_{j^*}(\cP)| \leq \alpha'$ except with probability $\beta'$.
\end{enumerate}
\end{proof}

This simple lemma yields an immediate corollary:

\begin{corollary}
Suppose that $M$ is $(\epsilon, 0)$-pointwise indistinguishable and $(\alpha,\beta)$-uniformly sample accurate. Then,
\[
\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A;S)}[\max_j |a_j - q_j(\cP)| \geq \alpha +\sqrt{\beta}+(e^\epsilon-1)] \leq \sqrt{\beta}
\]
i.e. it satisfies $(\alpha', \sqrt{\beta})$-uniform distributional accuracy for $\alpha' = \alpha +\sqrt{\beta}+(e^\epsilon-1)$.
\end{corollary}
\begin{proof}
We apply Theorem \ref{thm:transfer1} to $M$ with respect to the function $f_{\textrm{lift}}$ from Lemma \ref{lem:monitor}. By part 1 of Lemma \ref{lem:monitor}, $M$ is $(\alpha,\beta)$-sample accurate with respect to $f_{\textrm{lift}}$. Since it is also $(\epsilon,0)$-pointwise indistinguishable, Theorem \ref{thm:transfer1} allows us to conclude that $M$ is $(\alpha',\sqrt{\beta})$-distributionally accurate with respect to $f_{\textrm{lift}}$. Therefore, part 2 of Lemma \ref{lem:monitor} allows us to conclude that $M$ is $(\alpha',\sqrt{\beta})$-uniformly distributionally accurate.
\end{proof}


\ar{Trying an alternative way to finish the proof that gets a better dependence on $\beta$. Relies on a new observation: the posterior distributions $Q_\pi$ have to be well concentrated by Azuma's inequality. This actually also replaces our existing Lemma \ref{lem:exp}...}
\begin{lemma}\label{lem:tech'}
If $M$ is $(\epsilon,0)$-pointwise indistinguishable, then for any data distribution $\cP$,
\[
e^{-\epsilon} \Pr[\pirv = \pi | S_{< i} =\boldx_{< i}]  \le \Pr_{S \sim \cP^n}[\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}] \le e^\epsilon \Pr[\pirv = \pi | S_{< i} =\boldx_{< i}]
\]
\end{lemma}
\begin{proof}
\begin{align*}
\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] &= \sum_{\boldx_{>i}} \sum_{x_i} \Pr[S_i = x_i] \cdot \Pr[S_{>i} = \boldx_{>i}] \cdot \Pr[\pirv = \pi | S_{< i} =\boldx_{< i}, S_i = x_i, S_{>i} = \boldx_{>i}]\\
&\le e^\epsilon \sum_{\boldx_{>i}} \sum_{x_i} \Pr[S_i = x_i] \cdot \Pr[S_{>i} = \boldx_{>i}] \cdot \Pr[\pirv = \pi | S_{< i} =\boldx_{< i}, S_i = x, S_{>i} = \boldx_{>i}]\\
&= e^\epsilon \Pr_{S \sim \cP^n}[\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]
\end{align*}
The reverse inequality follows symmetrically.
\end{proof}

%\ar{Attempt 2}
\begin{lemma}\label{lem:tech2'}
If $M$ is $(\epsilon,0)$-pointwise indistinguishable, then for any data distribution $\cP$, if $S \sim \cP^n$ and any linear query $q$, with probability 1 over the draw of $\pi \sim \textrm{Interact}(M, A, f; S)$ for any $\eta > 0$:
$$\Pr_{S \sim Q_{\pi}}\left[|q(S)-q(\cP)| \geq (e^{\epsilon}-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \eta$$

\end{lemma}
\begin{proof}
Define the random variables $V_i = q(S_i) - \E[q(S_i) | S_{< i}]$, and let $X_i = \frac{1}{n}\sum_{j=1}^i V_j$. Then the sequence $0=X_0,X_1,\ldots,X_n$ forms a martingale and $|X_i - X_{i-1}| = \frac{1}{n}|V_i| \leq \frac{1}{n}$. We can therefore apply Azuma's inequality to conclude that:
\begin{equation}
\label{eq:azuma1}
\Pr\left[\left|\frac{1}{n}\sum_{i=1}^n q(S_i) - \frac{1}{n} \sum_{i=1}^n  \E[q(S_i) | S_{< i}]\right|\geq t \right] \leq 2\exp\left(\frac{-t^2n}{2}\right)
\end{equation}
Now fix any realization $\boldx$, and consider each term: $\E[q(S_i) | S_{< i} = \boldx_{<i}]$. We have:
\begin{eqnarray*}
\E_{S \sim Q_\pi}[q(S_i) | S_{< i} = \boldx_{<i}] &=&  \sum_x q(x)\cdot \Pr_{S \sim \cP^n}[S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] \\
&=& \sum_x q(x)\cdot \frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]\cdot \Pr_{S \sim \cP^n}[S_j = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } \\
&\leq& e^\epsilon \cdot \sum_x q(x)\cdot \Pr_{S \sim \cP^n}[S_i = x] \\
&=& e^\epsilon q(\cP)
\end{eqnarray*}
where the inequality follows from Lemma \ref{lem:tech'}. Symmetrically, $\E_{S \sim Q_\pi}[q(S_i) | S_{< i} = \boldx_{<i}]\geq e^{-\epsilon} q(\cP)$. Therefore we have that with probability $1$:
 $$e^{-\epsilon}q(\cP) \leq \frac{1}{n} \sum_{i=1}^n  \E[q(S_i) | S_{< i}]\leq e^\epsilon q(\cP).$$ Combining this with Equation \ref{eq:azuma1} gives us that for any $\eta > 0$, with probability $1-\eta$ when $S \sim Q_{\pi}$:
 $$q(S) \leq e^\epsilon q(\cP) + \sqrt{\frac{2\ln(2/\eta)}{n}} \ \ \textrm{and} \ \ q(S) \geq e^{-\epsilon} q(\cP) - \sqrt{\frac{2\ln(2/\eta)}{n}}$$
\end{proof}
This lets us prove a better transfer theorem:
\begin{theorem}\label{thm:better_transfer}
Suppose that $M$ is $(\epsilon,0)$-pointwise indistinguishable and $(\alpha,\beta)$-sample accurate with respect to $f$. Then for every $j$ indexing a linear query and any $\eta > 0$ it also satisfies:
$$\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A,f;S)}\left[|a_j - q_j(\cP)| \geq \alpha +(e^\epsilon-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \beta + \eta$$
i.e. it is $(\alpha', \beta')$-distributionally accurate with respect to $f$ for $\alpha' =  \alpha +(e^\epsilon-1)] + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta +\eta$.
\end{theorem}
\begin{proof}
Lemma \ref{lem:tech2'} and a triangle inequality proves the theorem.
\end{proof}


%\begin{lemma}[Method of Bounded Differences (Azuma's Inequality) \cite{DP09}]
%\label{lem:azuma}
%Let $S_1,\ldots,S_n$ be an arbitrary set of random variables, and let $q$ be a function satisfying the property that for each $i \in [n]$ there is a non-negative $c_i$ such that for every $\boldx$:
%$$\left|\E_S[f(S) | S_{\leq i}=\boldx_{\leq i}] - \E_S[f(S) | S_{\leq i}=\boldx_{\leq i-1}]\right| \leq c_i$$
%Then:
%$$\Pr_S[|f(S) - \E_S[f(S)]| \geq t] \leq 2\exp\left(-\frac{2t^2}{\sum_i c_i^2}\right)$$
%\end{lemma}
%
%\begin{lemma}
%If $M$ is $(\epsilon,0)$-pointwise indistinguishable, then for any data distribution $\cP$, if $S \sim \cP^n$ and any linear query $q$, with probability 1 over the draw of $\pi \sim \textrm{Interact}(M, A, f; S)$:
%$$\Pr_{S \sim Q_{\pi}}[|q(S)-q(Q_{\pi})| \geq O(\epsilon\cdot \sqrt{n\log 1/\delta})] \leq \delta$$ \ar{Would be nice to get a bound that was much better than this...}
%\end{lemma}
%\begin{proof}
%Our goal is to apply Azuma's inequality (Lemma \ref{lem:azuma}), and so we first verify that the random variables $S_1,\ldots,S_n$ satisfy the appropriate bounded differences condition. Fix any $\boldx$; For any index $i$, we can compute:
%\begin{eqnarray*}
%\E_{S \sim Q_\pi}[q(S) | S_{\leq i} = \boldx_{\leq i}] &=& \frac{1}{n}\sum_{j=1}^n \sum_x q(x)\cdot \Pr_{S \sim \cP^n}[S_j = x | \pirv=\pi, S_{\leq i} =\boldx_{\leq i}] \\
%&=& \frac{1}{n} \left(\sum_{j=1}^{i}q(\boldx_j) + \sum_{j=i+1}^n \sum_x q(x)\cdot \frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_j = x, S_{\leq i} = \boldx_{\leq i}]\cdot \Pr[S_j = x]}{\Pr[\pirv = \pi | S_{\leq i} =\boldx_{\leq i}] }\right) \\
%&\leq& \frac{1}{n} \left(\sum_{j=1}^{i}q(\boldx_j) + \sum_{j=i+1}^n \sum_x q(x)\cdot \frac{e^\epsilon \Pr_{S \sim \cP^n}[\pirv = \pi | S_j = x, S_{\leq i-1} = \boldx_{\leq i-1}]\cdot \Pr[S_j = x]}{e^{-\epsilon}\Pr[\pirv = \pi | S_{\leq i-1} =\boldx_{\leq i-1}] }\right) \\
%\end{eqnarray*}
%Similarly:
%$$\E_{S \sim Q_\pi}[q(S) | S_{\leq i} =\boldx_{\leq i}] =  \frac{1}{n} \left(\sum_{j=1}^{i-1}q(\boldx_j) + \sum_{j=i}^n \sum_x q(x)\cdot \frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_j = x, S_{\leq i-1} = \boldx_{\leq i-1}]\cdot \Pr[S_j = x]}{\Pr[\pirv = \pi | S_{\leq i-1} =\boldx_{\leq i-1}]}\right)$$
%Hence:
%$$\E_{S \sim Q_\pi}[q(S) | S_{\leq i} = \boldx_{\leq i}] -\E_{S \sim Q_\pi}[q(S) | S_{\leq i} =\boldx_{\leq i}] \leq$$
%$$\frac{1}{n}\left(q(\boldx_i) - \E_{S\sim Q_\pi}[q(S_i)| S_{\leq i-1} = \boldx_{\leq i-1}] +(e^{2\epsilon}-1)\sum_{j=i+1}^n \sum_x q(x)\cdot \frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_j = x, S_{\leq i-1} = \boldx_{\leq i-1}]\cdot \Pr[S_j = x]}{\Pr[\pirv = \pi | S_{\leq i-1} =\boldx_{\leq i-1}]}\right)\leq$$
%$$\frac{1 + (n-i)(e^{2\epsilon}-1)}{n}\approx 2\epsilon$$
%\ar{If $c_i = 2\epsilon$, then we get concentration $\approx \sqrt{n}\epsilon$, which isn't non-trivial until $\epsilon \ll 1/\sqrt{n}$...}
%\end{proof}


%\begin{theorem}
%Suppose that $M$ is $\epsilon$-differentially private and $(\alpha,\beta)$-uniform sample accurate. Then,
%\[\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A;S)}\left[ \max_{j} |a_j - q_j(\cP)| \geq \alpha +\sqrt{\beta}+(e^\epsilon-1)\right] \leq \sqrt{\beta}\]
%i.e. it achieves $(\alpha', \sqrt{\beta})$-uniform distributional accuracy where $\alpha' = \alpha +\sqrt{\beta}+(e^\epsilon-1)$.
%\end{theorem}
%\begin{proof}
%Instead of union bounding over all the queries, we'll ``lift" the bound we have for a single adaptively chosen query to the worst of a set of queries by considering a thought experiment. Assume we have a `Monitor' which knows the distribution $\cP$, which we'll denote as $\Theta_{\cP}$. Monitor $\Theta_{\cP}$ takes in a transcript $\pi$ and outputs the index whose query has the worst generalization error.
%\[
%\Theta_{\cP}(\pi) := \argmax_{j} |a_j - q_j(\cP)|.
%\]
%Note that this is only a thought experiment because it requires knowing the distribution $\cP$. Let $j^* = \Theta_{\cP}(\pi)$. Because $\Theta_\cP$ doesn't look at the dataset $S$, $j^*$ is $\epsilon$-differentially private with respect to $S$. \cj{Should make it more clear that this monitor part doesn't undo lemma \ref{lem:exp}}
%
%\begin{lemma}
%\label{lem:monitor_posterior_accuracy}
%Given same conditions as the theorem,
%\[
%\Pr_{S \sim \cP^n, \pirv \sim I(S)}\left[|q_{j^*} (Q_\pi) - a_{j^*} | \ge \alpha + \sqrt{\beta}\right] \le \sqrt{\beta}
%\]
%\end{lemma}
%\begin{proof}
%By the guarantee of $(\alpha,\beta)$-uniform sample accuracy and the Bayesian resampling Lemma \ref{lem:resamp},
%\begin{align*}
%&\Pr_{S \sim \cP^n, \pirv \sim I(S)} \left[\Pr_{S' \sim Q_{\pirv}}\left[ |q_{j^*}(S') - a_{j^*}| \geq \alpha \right]\right]\\
%&=\E_{S \sim \cP^n, \pirv \sim I(S)} \left[\Pr_{S' \sim Q_{\pirv}}\left[ |q_{j^*}(S') - a_{j^*}| \geq \alpha \right]\right]\\
%&=\E_{S \sim \cP^n, \pirv \sim I(S), S' \sim Q_{\pirv}} \left[ |q_{j^*}(S') - a_{j^*}| \geq \alpha \right]\\
%&= \E_{S \sim \cP^n} \left[ \Pr_{\pirv \sim I(S)}\left[|q_{j^*}(S) - a_{j^*}| \geq \alpha \right] \right] \\
%&\le \E_{S \sim \cP^n} \left[ \beta \right] \\
%&\le \beta.
%\end{align*}
%Let $E(\pirv,S')$ be the event that $|q_{j^*}(S') - a_{j^*}| \geq \alpha$. By Markov's inequality,
%\[
%\Pr_{S \sim \cP^n,\pirv \sim I(S)}\left[\Pr_{S' \sim Q_{\pirv}}[E(\pirv,S')] \geq \sqrt{\beta}\right] \leq \sqrt{\beta}.
%\]
%Let $G = \{\pi \in \pispace : \Pr_{S' \sim Q_{\pi}}[E(\pi,S')] \leq \sqrt{\beta}\}$ (so $\Pr[\pirv \in G] \geq 1-\sqrt{\beta}$). For any $\pi \in G$, we must have:
%%$$(1-\sqrt{\beta})(a-\alpha)\leq \E_{S' \sim Q_{\pi}}[\frac{1}{n}\sum_{i=1}^n q_j(S'_i)] \leq (1-\sqrt{\beta})(a+\alpha) + \sqrt{\beta}$$
%\begin{eqnarray*}
%q_{j^*} (Q_\pi) &=& \E_{S' \sim Q_{\pi}}[q_{j^*}(S')] \\
%&=& \underbrace{\E_{S' \sim Q_{\pi}}[q_{j^*}(S')|E(\pi,S')]}_{\le 1} \cdot \underbrace{\Pr_{S' \sim Q_{\pi}} [E(\pi,S')]}_{\le \sqrt{\beta}} + \underbrace{\E_{S' \sim Q_{\pi}}[q_{j^*}(S')|\neg E(\pi,S')]}_{\le a_{j^*} + \alpha} \cdot \underbrace{\Pr_{S' \sim Q_{\pi}} [\neg E(\pi,S')]}_{\le 1} \\
%&\leq& a_{j^*}+ \alpha + \sqrt{\beta}
%\end{eqnarray*}
%Similarly:
%\begin{eqnarray*}
%q_{j^*} (Q_\pi) &=& \E_{S' \sim Q_{\pi}}[q_{j^*}(S')] \\
%&\geq& \underbrace{\E_{S' \sim Q_{\pi}}[q_{j^*}(S')|\neg E(\pi,S')]}_{\ge a_{j^*} - \alpha} \cdot \underbrace{\Pr_{S' \sim Q_{\pi}} [\neg E(\pi,S')]}_{\ge 1-\sqrt{\beta}} \\
%&\ge& (a_{j^*}-\alpha)(1-\sqrt{\beta}) \\
%&\geq& a_{j^*}-\alpha -\sqrt{\beta}
%\end{eqnarray*}
%We therefore have that for $\pi \in G$,
%\[
%| q_{j^*} (Q_\pi) - a_{j^*} | \le \alpha + \sqrt{\beta}
%\]
%Since $\Pr[\pirv \in G] \geq 1-\sqrt{\beta}$, this proves the lemma.
%\end{proof}
%
%Finally, combining Lemma \ref{lem:exp} and Lemma \ref{lem:monitor_posterior_accuracy}, we have that with probability $1-\sqrt{\beta}$ over the randomness of $S$ and $\pirv$,
%\begin{align*}
%\max_{j} |a_j - q_j(\cP)| = \left|a_{j^*} - q_{j^*}(\cP)\right| &\le \left|a_{j^*} - q_{j^*}(Q_{\pi}) \right| + \left|q_{j^*}(Q_{\pi})  - q_{j^*}(\cP) \right|\\
%&\le \alpha + \sqrt{\beta} + (e^\epsilon - 1)
%\end{align*}
%
%\end{proof}
\fi














\subsection{Generalization to $(\epsilon,\delta)$-Differential Privacy}
\label{sec:delta2}

\iffalse
%The proof generalizes to $(\epsilon,\delta)$-pointwise indistinguishability with the same basic outline as the warmup argument for $(\epsilon,0)$-pointwise indistinguishability. Here we generalize the lemmas we need.
%First we prove a technical lemma that is the analogue of Lemma \ref{lem:tech1} for $(\epsilon,\delta)$-pointwise indistinguishability:

\begin{lemma}
\label{lem:tech2}
For any $x \in \cX$ and $i \in [n]$, if $M$ is $(\epsilon,\delta)$-pointwise indistinguishable:
\begin{itemize}
\item with probability $1-\sqrt{\delta}$ over $\pi \sim \pirv$: $\Pr[\pirv = \pi] \leq \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr[\pirv = \pi | S_i = x]$.
\item with probability $1-\sqrt{\delta}$ over $\pi \sim \pirv|S_i=x$: $ \Pr[\pirv = \pi | S_i = x] \leq \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr[\pirv = \pi]$.
\end{itemize}
% then with probability at least $1-\sqrt{\delta} - \delta^{1/4}$ over the selection of $\pi$:
%\[e^{-\epsilon} \left( 1 - \left( \frac{e^\epsilon \sqrt{\delta}}{1 - \sqrt{\delta}} + 1\right) \delta^{1/4} \right) \Pr[\pi | S_i = x] \leq \Pr[\pi] \leq \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr[\pi | S_i = x]\]
\end{lemma}
\begin{proof}
In this proof, we will use the following definitions of bad and good sets of transcripts:
\begin{definition}
We define the \emph{bad and good} sets of transcripts $\pi$ given a pair of data points $x,x'$ and a dataset $\boldx_{-i} \in \cX^{n-1}$ at level $\epsilon \geq 0$ as:
$$G(\boldx_{-i},x,x',\epsilon) = \{\pi: e^{-\epsilon} \leq \frac{\Pr[\textrm{Interact}(M, A; \boldx_{-i},x) = \pi]}{\Pr[\textrm{Interact}(M, A; \boldx_{-i},x') = \pi]} \leq e^{\epsilon}\}$$
$$B(\boldx_{-i},x,x',\epsilon) = \pispace \setminus G(\boldx_{-i},x,x',\epsilon) =  \{\pi : \pi \not\in G(\boldx_{-i},x,x',\epsilon)\}$$
\end{definition}
Note that by the definition of $(\epsilon,\delta)$-pointwise indistinguishability, it is immediate that for any $\boldx_{-i}, x, x'$: $\Pr[\pirv \in B(\boldx_{-i},x,x',\epsilon) | \boldx_{-i}, x'] \leq \delta$.

We prove each part of the lemma in turn. First, for any transcript $\pi$, we have:
\begin{eqnarray*}
\Pr[\pirv = \pi] &=& \sum_{(\boldx_{-i},x')}\Pr[S = (\boldx_{-i},x')] \Pr[\pirv = \pi | S = (\boldx_{-i},x')] \\
&=& \sum_{(\boldx_{-i},x'): \pi \in G(\boldx_{-i},x,x',\epsilon)}\Pr[S= (\boldx_{-i},x')] \Pr[\pirv = \pi | S= (\boldx_{-i},x')]\\
&+& \sum_{(\boldx_{-i},x'): \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S= (\boldx_{-i},x')] \Pr[\pirv = \pi | S= (\boldx_{-i},x')]  \\
&\leq& \sum_{(\boldx_{-i},x'): \pi \in G(\boldx_{-i},x,x',\epsilon)}\Pr[S= (\boldx_{-i},x')] \cdot e^{\epsilon} \Pr[\pirv = \pi | S= (\boldx_{-i},x)] \\
&+& \sum_{(\boldx_{-i},x'):\pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S= (\boldx_{-i},x')] \Pr[\pirv = \pi | S= (\boldx_{-i},x')]  \\
&\leq& e^\epsilon \Pr[\pirv = \pi|S_i = x] +  \sum_{(\boldx_{-i},x'): \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S= (\boldx_{-i},x')] \Pr[\pirv = \pi | S= (\boldx_{-i},x')] \\
&=& e^\epsilon \Pr[\pirv = \pi|S_i = x] + \sum_{(\boldx_{-i},x'): \pi \in B(\boldx_{-i},x,x',\epsilon)} \Pr[\pirv = \pi] \Pr[S = (\boldx_{-i},x')  | \pirv = \pi] \\
&=&e^\epsilon \Pr[\pirv = \pi|S_i = x] + \Pr[\pirv = \pi] \cdot \Pr_{(S_{-i},x') \sim Q_\pi}[\pi \in B(S_{-i},x,x',\epsilon)]
\end{eqnarray*}

It remains to show that $\Pr_{(S_{-i},x') \sim Q_\pi}[\pi \in B(S_{-i},x,x',\epsilon)] \leq \sqrt{\delta}$ with probability at least $1-\sqrt{\delta}$ over the selection of $\pi \sim \pirv$. This follows from Markov's inequality. By the guarantee of $(\epsilon,\delta)$-pointwise indistinguishability, and the Bayesian resampling lemma (Lemma \ref{lem:resamp}) we have that:
\begin{eqnarray*}
\delta &\geq& \E_{(S_{-i},x') \sim \cP^n}[\Pr_{\pi \sim \pirv} [\pi \in B(S_{-i},x,x',\epsilon)]] \\
&=& \E_{\pi \sim \Pi}[\Pr_{(S_{-i},x') \sim Q_\pi}[\pi \in B(S_{-i},x,x',\epsilon)]]
\end{eqnarray*}

By Markov's inequality, we therefore have that:
$$\Pr_{\pi \sim \pirv}[\Pr_{(S_{-i},x') \sim Q_\pi}[\pi \in B(S_{-i},x,x',\epsilon)] \geq \sqrt{\delta}]\leq \sqrt{\delta}$$

In the reverse direction:
\begin{align*}
&\Pr[\pirv = \pi|S_i = x] \\
&= \sum_{(\boldx_{-i},x')}\Pr[S_{-i} = \boldx_{-i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{-i},x)] \\
&=\sum_{(\boldx_{-i},x'): \pi \in G(\boldx_{-i},x,x',\epsilon)}\Pr[S_{-i} = \boldx_{-i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{-i},x)] \\
&+ \sum_{(\boldx_{-i},x'): \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S_{-i} = \boldx_{-i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{-i},x)] \\
&\leq \sum_{(\boldx_{-i},x'): \pi \in G(\boldx_{-i},x,x',\epsilon)}\Pr[S_{-i} = \boldx_{-i}]\cdot\Pr[S_i = x']\cdot e^\epsilon \Pr[\pirv = \pi| S = (\boldx_{-i},x')] \\
&+ \sum_{(\boldx_{-i},x'): \pi \in B(\boldx_{-i},x,x',\epsilon) }\Pr[S_{-i} = \boldx_{-i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{-i},x)] \\
&\leq e^\epsilon \Pr[\pirv = \pi] +  \sum_{(\boldx_{-i},x') : \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S_{-i} =\boldx_{-i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{-i},x)] \\
&=  e^\epsilon \Pr[\pirv = \pi] +  \sum_{(\boldx_{-i},x') : \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S_i = x']\cdot \Pr[S_{-i} = \boldx_{-i}]\cdot \frac{\Pr[S_{-i} = \boldx_{-i}| \pirv = \pi,S_i=x]\cdot \Pr[\pirv = \pi |S_i = x]}{\Pr[S_{-i} = \boldx_{-i}|S_i = x]} \\
&= e^\epsilon \Pr[\pirv = \pi] + \Pr[\pirv = \pi|S_i = x]\cdot \sum_{(\boldx_{-i},x') : \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S_i = x']\cdot \Pr[S_{-i} = \boldx_{-i}| \pirv = \pi,S_i=x]
\end{align*}

Let $f(\pi,x) := \sum_{(\boldx_{-i},x') : \pi \in B(\boldx_{-i},x,x',\epsilon)}\Pr[S_i = x']\cdot \Pr[S_{-i} = \boldx_{-i}|\pirv = \pi,S_i=x] $. We have that
\begin{align*}
&\E_{\pi \sim \pirv| S_i = x} \left[ f(\pi,x) \right]  \\
&= \sum_{\pi} \Pr [\pirv = \pi | S_i =x] \sum_{(\boldx_{-i},x')}  \Pr[S_i = x'] \Pr[S_{-i} = \boldx_{-i}|\pirv = \pi,S_i=x] \1 [\pi \in B(\boldx_{-i},x,x',\epsilon)] \\
&= \sum_{\pi} \sum_{(\boldx_{-i},x')} \Pr [\pirv = \pi| S_i =x] \Pr[S_i = x'] \frac{\Pr[\pirv = \pi | S=(\boldx_{-i},x)] \Pr [S_{-i} = \boldx_{-i} | S_i = x]}{\Pr [\pirv = \pi | S_i = x] } \1 [\pi \in B(\boldx_{-i},x,x',\epsilon)] \\
&=  \sum_{\pi} \sum_{(\boldx_{-i},x')} \Pr[S = (\boldx_{-i}, x')] \Pr[\pirv = \pi | S = (\boldx_{-i}, x)] \1 [\pi \in B(\boldx_{-i},x,x',\epsilon)]  \\
&=  \sum_{(\boldx_{-i},x')} \Pr[S = (\boldx_{-i}, x')] \sum_{\pi} \Pr[\pirv = \pi | S = (\boldx_{-i}, x)] \1 [\pi \in B(\boldx_{-i},x,x',\epsilon)]  \\
&= \E_{(S_{-i},x') \sim \cP^n} \left[ \Pr_{\pi \sim \pirv} \left[ \pi \in B(S_{-i},x,x',\epsilon) | S_{-i}, x \right] \right] \\
&\le \delta
\end{align*}

Hence, by Markov's inequality,
$$
\Pr_{\pi \sim \pirv | S_i = x} \left[ f(\pi,x) > \sqrt{\delta} \right] \le \sqrt{\delta}
$$
completing the proof.
%Let $f(\pi,x) := \sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[x']\cdot \Pr[S_{-i}|\pi,S_i=x] $. Define
%$
%\Pi_1 = \left\{ \pi: \Pr \left[\pi \right] \le \frac{e^\epsilon}{1 - \sqrt{\delta}} \Pr[\pi|S_i = x] \right\}
%$
%and recall from the first part of this Lemma that $\Pr_\pi \left[ \pi \notin \Pi_1 \right] \le \sqrt{\delta}$. We have that
%\begin{align*}
%\E_\pi \left[ f(\pi,x) \right] &= \E_\pi \left[ f(\pi,x) \1 [\pi \in \Pi_1 ]\right] + \E_\pi \left[ f(\pi,x) \1 [\pi \notin \Pi_1 ]\right] \\
%&\le \E_\pi \left[ f(\pi,x) \1 [\pi \in \Pi_1 ]\right] + \sqrt{\delta} \\
%&= \sum_{\pi \in \Pi_1} \sum_{(S_{-i},x')} \Pr [\pi] \Pr[x'] \Pr[S_{-i}|\pi,S_i=x] \1 [\pi \in B(S_{-i},x,x',\epsilon)] + \sqrt{\delta} \\
%&= \sum_{\pi \in \Pi_1} \sum_{(S_{-i},x')} \Pr [\pi] \Pr[x'] \frac{\Pr[\pi | S_{-i},S_i = x] \Pr [S_{-i} | S_i = x]}{\Pr [\pi | S_i = x] } \1 [\pi \in B(S_{-i},x,x',\epsilon)] + \sqrt{\delta}\\
%&= \sum_{\pi \in \Pi_1} \sum_{(S_{-i},x')} \frac{\Pr [\pi]}{\Pr [\pi | S_i = x] } \Pr[x'] \Pr [S_{-i}]  \Pr[\pi | S_{-i}, x] \1 [\pi \in B(S_{-i},x,x',\epsilon)] + \sqrt{\delta} \\
%&\le \frac{e^\epsilon}{1 - \sqrt{\delta}} \sum_{\pi} \sum_{(S_{-i},x')} \Pr[S_{-i}, x'] \Pr[\pi | S_{-i}, x] \1 [\pi \in B(S_{-i},x,x',\epsilon)] + \sqrt{\delta} \\
%&=  \frac{e^\epsilon}{1 - \sqrt{\delta}} \sum_{(S_{-i},x')} \Pr[S_{-i}, x'] \sum_{\pi} \Pr[\pi | S_{-i}, x] \1 [\pi \in B(S_{-i},x,x',\epsilon)] + \sqrt{\delta} \\
%&= \frac{e^\epsilon}{1 - \sqrt{\delta}} \E_{(S_{-i},x') \sim \cP^n} \left[ \Pr_\pi \left[ \pi \in B(S_{-i},x,x',\epsilon) | S_{-i}, x \right] \right] + \sqrt{\delta} \\
%&\le \frac{e^\epsilon}{1 - \sqrt{\delta}} \cdot \delta + \sqrt{\delta}
%\end{align*}
%By Markov's inequality we have that:
%$$
%\Pr_{ \pi } \left[ f(\pi,x) \ge   \left( \frac{e^\epsilon \sqrt{\delta}}{1 - \sqrt{\delta}} + 1\right) \delta^{1/4} \right] \le \delta^{1/4}
%$$
%and therefore, with probability at least $1 - \delta^{1/4}$ over the selection of $\pi$:
%$$
%\Pr[\pi|S_i = x] \le e^\epsilon \Pr[\pi] + \Pr[\pi|S_i = x]\cdot  \left( \frac{e^\epsilon \sqrt{\delta}}{1 - \sqrt{\delta}} + 1\right) \delta^{1/4}
%$$
%completing the proof.

%Given $\pi$, $x$, and $i$, $Q_{\pi,x,i} (S_{-i}, x') := \Pr[x']\cdot \Pr[S_{-i}|\pi,S_i=x]$ forms a distribution over the data space. We are interested in bounding $\Pr_{(S_{-i},x') \sim Q_{\pi,x,i} } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right]$. Let for now the distribution over the transcripts be $Q (\pi) = \Pr \left[ \pi | S_i = x\right]$ and assume the conditional distribution of $S=(S_i,x')$ given $\pi$ is $Q(S | \pi) = Q_{\pi,x,i} (S_{-i}, x')$. Let's look at the distribution imposed on the joint $(\pi,S)$:
%$$
%Q(\pi, S) = Q(S | \pi) \cdot Q(\pi) = \Pr[x'] \Pr[S_{-i}|\pi,S_i=x] \cdot \Pr \left[ \pi | S_i = x\right]
%$$
%The marginal distribution of $S=(S_{-i},x')$ for the joint distribution $Q(\pi, S)$:
%$$
%Q(S) = \sum_{\pi} Q(\pi, S) = \Pr[x'] \Pr[S_{-i}| S_i=x] = \Pr \left[ S \right]
%$$
%which means $S \sim \cP^n$. Now let's find $Q(\pi | S)$:
%$$
%Q(\pi | S) = \frac{Q(\pi, S)}{Q(S)} = \frac{\Pr \left[ \pi | S_i = x\right] \Pr[S_{-i}|\pi,S_i=x] }{\Pr[S_{-i}]} = \Pr \left[ \pi | S_{-i}, x\right]
%$$
%We therefore have that
%\begin{eqnarray*}
%\E_{\pi \sim Q(\pi)} \left[ \Pr_{(S_{-i},x') \sim Q(S|\pi) } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \right] &=& \Pr_{(\pi,S) \sim Q(\pi,S)} \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \\
%&=& \E_{S \sim Q(S)} \left[ \Pr_{\pi \sim Q(\pi |S) } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \right] \\
%&=& \E_{(S_{-i},x') \sim \cP^n } \left[ \Pr_{\pi \sim \Pr [\pi | S_{-i}, x] } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \right] \\
%&=& \E_{(S_{-i},x') \sim \cP^n } \left[ \Pr_{\pi \sim \Pr [\pi | S_{-i}, x] } \left[ \pi \in B \left( S_{-i}, x', x, \epsilon \right) \right] \right] \\
%&\le& \delta
%\end{eqnarray*}
%Because $\Pr_{\pi \sim \Pr [\pi | S_{-i}, x] } \left[ \pi \in B \left( S_{-i}, x', x, \epsilon \right) \right] \le \delta$ for all $(S_{-i}, x')$. But notice we want the above expectation with respect to the unconditional distribution of $\pi$, i.e., $\Pr [\pi]$. Recall from the first part of the Lemma that with probability at least $1 - \sqrt{\delta}$ over $\pi$, $\Pr [\pi] \le \frac{e^\epsilon}{1 - \sqrt{\delta}} \Pr [\pi | S_i = x]$. Hence
%\begin{align*}
%&\E_{\pi \sim \Pr[\pi]} \left[ \Pr_{(S_{-i},x') \sim Q(S|\pi) } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \right] \\
%&\le \frac{e^\epsilon}{1 - \sqrt{\delta}} \cdot \E_{\pi \sim Q(\pi)} \left[ \Pr_{(S_{-i},x') \sim Q(S|\pi) } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \right] + \sqrt{\delta} \\
%&\le \frac{e^\epsilon}{1 - \sqrt{\delta}} \cdot \delta + \sqrt{\delta}
%\end{align*}
%%\begin{eqnarray*}
%%\E_{S' \sim \cP^n, \pi \sim I(S')} \left[ \Pr_{(S_{-i},x') \sim Q_{\pi,x} } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \right] &=& \Pr_{\substack{S' \sim \cP^n, \pi \sim I(S') \\ x' \sim \cP, S_{-i} \sim \cP_{\pi,x}}} \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \\
%%&=& \E_{S \sim \text{some distribution}} \left[ \Pr_{\pi \sim I(S)} \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \vert S \right] \right] \\
%%&\le& \delta
%%\end{eqnarray*}
%%\cj{We may need to reweigh the original distribution, but it doesn't matter because once we fix $S$, probability of choosing some bad $\pi$ is still bounded}
%Finally, Markov's inequality would then imply with probability at least $1-\delta^{1/4}$ over the selection of $\pi$:
%$$
%\Pr_{(S_{-i},x') \sim Q_{\pi,x,i} } \left[ \pi \in B \left( S_{-i}, x, x', \epsilon \right) \right] \le \left( \frac{e^\epsilon \sqrt{\delta}}{1 - \sqrt{\delta}} + 1\right) \delta^{1/4}
%$$
%Therefore, with probability at least $1-\delta^{1/4}$ over the selection of $\pi$:
%$$
%\Pr \left[\pi \right] \ge e^{-\epsilon} \left( 1 - \left( \frac{e^\epsilon \sqrt{\delta}}{1 - \sqrt{\delta}} + 1\right) \delta^{1/4} \right) \Pr[\pi|S_i = x]
%$$
%completing the proof.
%\ar{Need to figure out how to continue. Alternate approach follows}
%\fi
%In the reverse direction:
%\begin{eqnarray*}
%\Pr[\pi] &=& \sum_{S = (S_{-i},x')}\Pr[S]\cdot \Pr[\pi | S] \\
%&=& \sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | S] + \sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | S] \\
%&\geq&\sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot e^{-\epsilon}\Pr[\pi | (S_{-i},x)] + \sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | S] \\
%&\geq&\sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot e^{-\epsilon}\Pr[\pi | (S_{-i},x)] \\
%&=& e^{-\epsilon} \left( \Pr[\pi|S_i = x] -  \sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | (S_{-i},x)] \right)
%\end{eqnarray*}
%We've shown that with probability $1-\sqrt{\delta}$ over the draw of $\pi$,  $\sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | (S_{-i},x)] \leq \Pr[\pi] \sqrt{\delta} $ \ar{Er, not quite, right? We showed this for a different expression: $\sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | (S_{-i},x')] \leq \Pr[\pi] \sqrt{\delta}$. -- i.e. the $x'$ has been swapped with an $x$ here.} Hence:

%\begin{eqnarray*}
%\Pr[\pi] \geq e^{-\epsilon} \left( \Pr[\pi|S_i = x] -  \sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | (S_{-i},x)] \right) \geq \\
 % e^{-\epsilon} \left( \Pr[\pi|S_i = x] - \Pr[\pi]\sqrt{\delta}\right)
%\end{eqnarray*}


%\cj{Here's my attempt}
%Note that because for any $S_{-i},x,x'$, $\Pr(\pi \in B(S_{-i},x,x',\epsilon ) | S_{-i}, x) \le \delta$, we have for any $S_{-i},x,x'$
%\[
%\Pr(\pi \in G(S_{-i},x,x',\epsilon ) | S_{-i}, x) \ge 1- \delta.
%\]
%\begin{eqnarray*}
%\Pr[\pi] &=& \sum_{S = (S_{-i},x')}\Pr[S]\cdot \Pr[\pi | S] \\
%&=& \sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | S] + \sum_{(S_{-i},x') : \pi \in B(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | S] \\
%&\ge& \sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot \Pr[\pi | S]\\
%&\ge& \sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot e^{-\epsilon} \Pr[\pi | S_{-i}, x]\\
%&\ge& \sum_{(S_{-i},x') : \pi \in G(S_{-i},x,x',\epsilon)}\Pr[S]\cdot e^{-\epsilon} \Pr[\pi | S_{-i}, x]\\
%\end{eqnarray*}
\end{proof}




%Using Lemma \ref{lem:tech2}, we prove an analogue of Lemma \ref{lem:exp}.

\begin{lemma}
\label{lem:exp2}
Suppose $Q_\pi^1 = Q_\pi^2 = \ldots = Q_\pi^n := \cP_\pi$ (this means the data set $S$ is unordered and is equivalent to saying: $\Pr \left[ \pi | S_1 = x\right] = \Pr \left[ \pi | S_i = x\right]$ for all $i$) \ar{Probably this should just be a modeling assumption we make in the prelims, not here.}. We therefore use notations $\Pr \left[ \pi | x \right] := \Pr \left[ \pi | S_1 = x\right]$ and $\Pr \left[ x | \pi \right] := \Pr \left[ S_1 = x | \pi \right]$ in this setting. If $M$ is $(\epsilon,\delta)$-pointwise indistinguishable, then for any data distribution $\cP$ and any linear query $q$, if $S \sim \cP^n$, with probability $1-2\delta^{1/4}$ over the draw of $\pi \sim \textrm{Interact}(M, A; S)$:
$$\left|q(Q_\pi) - q(\cP)\right| \leq \frac{e^{\epsilon}}{1-\sqrt{\delta}} - 1 + \delta^{1/4}$$
%$$\left|\E_{S \sim Q_\pi}[\frac{1}{n}\sum_{i=1}^n q(S_i)] -  \E_{S \sim \cP^n}[\frac{1}{n}\sum_{i=1}^n q(S_i)]\right|  \leq \max(e^\epsilon -1, 1-e^{-\epsilon}) = e^\epsilon-1$$
\end{lemma}
\begin{proof}

%For simplicity, let $K(\epsilon, \delta) :=  1 - \left( \frac{e^\epsilon \sqrt{\delta}}{1 - \sqrt{\delta}} + 1\right) \delta^{1/4}$. Notice $K(\epsilon, \delta) \ge 1 - 2 \delta^{1/4}$ for reasonable values of $\epsilon,\delta$ \saeed{Shall we assume this always holds?}. In this proof, we will use the following definition of bad and good \emph{data points} with respect to a transcript $\pi$:
%\begin{definition}
%For a given $\epsilon,\delta$, we define the \emph{bad and good} sets of datapoints $x$ given a transcript $\pi$ as:
%$$G (\pi,\epsilon,\delta) = \left\{x : e^{-\epsilon} K(\epsilon, \delta) \Pr[\pi | x]  \leq \Pr[\pi] \leq \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr[\pi | x] \right\}$$
%$$B (\pi,\epsilon,\delta) = \cX\setminus G (\pi,\epsilon,\delta) =  \{x : x \not\in G (\pi,\epsilon,\delta)\}$$
%\end{definition}
Define the following events for a given $\epsilon, \delta$, and $\pi$:
$$
G_u (\pi, \epsilon, \delta) = \left\{x : \Pr[\pi] \leq \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr[\pi | x] \right\}
$$
$$
G_l (\pi, \epsilon, \delta) = \left\{x : \Pr[\pi | x]  \leq \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr[\pi] \right\}
$$
%First, we observe that for most transcripts $\pi$, a randomly selected point $x \sim \cP_\pi$ is unlikely to fall into the bad set:
\begin{claim}\label{bpi}
We have that:
\begin{itemize}
\item With probability $1 - \delta^{1/4}$ over the selection of $\pi$: $\Pr_{x \sim \cP}[x \notin G_u (\pi,\epsilon,\delta)] \le \delta^{1/4}$
\item With probability $1 - \delta^{1/4}$ over the selection of $\pi$: $\Pr_{x \sim \cP_\pi}[x \notin G_l (\pi,\epsilon,\delta)] \leq \delta^{1/4}$
\end{itemize}
\end{claim}

\begin{proof}
Observe that Lemma \ref{lem:tech2} implies:
$$
\E_\pi \left[ \Pr_{x \sim \cP}[x \notin G_u (\pi,\epsilon,\delta)] \right] = \E_{x \sim \cP} \left[ \Pr_{\pi}[x \notin G_u (\pi,\epsilon,\delta)] \right] \le \sqrt{\delta}
$$
$$
\E_\pi \left[ \Pr_{x \sim \cP_\pi }[x \notin G_l (\pi,\epsilon,\delta)] \right] = \E_{x \sim \cP} \left[ \Pr_{\pi | x }[x \notin G_l (\pi,\epsilon,\delta)] \right] \le \sqrt{\delta}
$$
Markov's inequality completes the proof.
\end{proof}

%Let $\Pi_x = \left\{ \pi: \Pr [ \pi | x ] \le e^\epsilon K^{-1} (\epsilon, \delta) \Pr [\pi]\right\}$ and recall that for all $x$, $\Pr [ \pi \notin \Pi_x ] \le \delta^{1/4}$.
%\begin{align*}
%\E_\pi \left[ \Pr_{x \sim \cP_\pi} \left[ x \in B (\pi,\epsilon,\delta)\right] \right] &= \E_{x \sim \cP} \left[ \Pr_{\pi|x} \left[ x \in B (\pi,\epsilon,\delta)\right] \right] \\
%&= \E_{x \sim \cP} \left[ \E_{\pi|x} \left[ \1[ x \in B (\pi,\epsilon,\delta)] \1[\pi \in \Pi_x] \right] \right] + \E_{x \sim \cP} \left[ \E_{\pi|x} \left[ \1[ x \in B (\pi,\epsilon,\delta)] \1[\pi \notin \Pi_x] \right] \right] \\
%&\le \E_{x \sim \cP} \left[ \E_{\pi|x} \left[ \1[ x \in B (\pi,\epsilon,\delta)] \1[\pi \in \Pi_x] \right] \right] + \E_{x \sim \cP} \left[ \Pr_{\pi|x} \left[  \pi \notin \Pi_x \right] \right] \\
%&\le e^\epsilon K^{-1} (\epsilon, \delta) \cdot \E_{x \sim \cP} \left[ \Pr_{\pi} \left[ x \in B (\pi,\epsilon,\delta)  \right] \right] + \E_{x \sim \cP} \left[ \Pr_{\pi|x} \left[  \pi \notin \Pi_x \right] \right] \\
%&\le \left( \sqrt{\delta} + \delta^{1/4} \right) e^\epsilon K^{-1} (\epsilon, \delta) + \E_{x \sim \cP} \left[ \Pr_{\pi|x} \left[  \pi \notin \Pi_x \right] \right]
%\end{align*}
%We only need to show that for every $x$, $\Pr_{\pi|x} \left[  \pi \notin \Pi_x \right] \le \sqrt{\delta}$. Fix some $x$. We showed in the previous Lemma that
%$$
%\Pr[\pi| S_i = x] \le e^\epsilon \Pr[\pi] + \Pr[\pi| S_i = x]\cdot f(\pi,x)
%$$
%where $f(\pi,x) = \sum_{(S_{-i},x')}\Pr[x']\cdot \Pr[S_{-i}|\pi,S_i=x] \1[\pi \in B(S_{-i},x,x',\epsilon) ]$. But
%\begin{align*}
%\E_{\pi | x} \left[ f(\pi,x) \right] &= \sum_{\pi} \sum_{(S_{-i},x')} \Pr [\pi | S_i = x] \Pr[x'] \Pr[S_{-i}|\pi,S_i=x] \1 [\pi \in B(S_{-i},x,x',\epsilon)] \\
%&= \sum_{\pi} \sum_{(S_{-i},x')} \Pr [\pi | S_i=x ] \Pr[x'] \frac{\Pr[\pi | S_{-i},S_i = x] \Pr [S_{-i} | S_i = x]}{\Pr [\pi | S_i = x] } \1 [\pi \in B(S_{-i},x,x',\epsilon)]\\
%&= \sum_{(S_{-i},x')} \Pr [S_{-i}, x'] \sum_{\pi} \Pr[\pi | S_{-i},S_i = x] \1 [\pi \in B(S_{-i},x,x',\epsilon)] \\
%&=\E_{(S_{-i},x') \sim \cP^n} \left[ \Pr_\pi \left[ \pi \in B(S_{-i},x,x',\epsilon) | S_{-i}, x \right] \right] \\
%&\le \delta
%\end{align*}
%which implies by Markov's inequality that with probability at least $1-\sqrt{\delta}$ over the conditional distribution $\pi | x$, $f(\pi,x) \le \sqrt{\delta}$. Consequently, with probability at least $1-\sqrt{\delta}$ over the conditional distribution $\pi | x$,
%$$
%\Pr [ \pi | x] \le \frac{e^\epsilon}{1-\sqrt{\delta}} \Pr [\pi] \le e^\epsilon K^{-1} (\epsilon, \delta) \Pr [\pi]
%$$
%
%Lemma \ref{lem:tech2} gives us that for \emph{every} $x$, $\Pr_{\pi}[x \in B(\pi,\epsilon,\delta)] \leq \sqrt{\delta} + \delta^{1/4}$. This guarantee therefore also holds over the randomness of $x$: in particular this implies that: $\E_{\pi}[\Pr_{x \sim \cP_\pi}[x \in  B(\pi,\epsilon,\delta)] ]\leq \sqrt{\delta} + \delta^{1/4}$. The claim then follows from Markov's inequality. \saeed{not clear enough}

%\sn{Stopped here: I think we need the above claim with $Q_\pi$ instead of $P$ to finish the argument and bound the RHS by $\delta^{1/4}$}\ar{Agree this seems to be the claim we need with the current outline. Or maybe there is another path to where we want to go..}

Let's prove Lemma \ref{lem:exp2}. First:
\begin{eqnarray*}
q(Q_\pi) &=& \E_{S \sim Q_\pi}[\frac{1}{n}\sum_{i=1}^n q(S_i)] \\
&=& \frac{1}{n} \sum_{i=1}^n \E_{S \sim Q_\pi}[q(S_i)] \\
&=& \frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \Pr_{S \sim Q_\pi}[S_i = x] \\
&=& \frac{1}{n} \sum_{i=1}^n \sum_{x \in \cX} q(x) \cdot \Pr_{S \sim \cP^n}[S_i = x | \pi] \\
&=& \frac{1}{n} \sum_{i=1}^n \left(\sum_{x \in G_l (\pi,\epsilon,\delta)} q(x) \cdot \Pr_{S \sim \cP^n}[S_i = x | \pi] + \sum_{x \notin G_l (\pi,\epsilon,\delta)} q(x) \cdot \Pr_{S \sim \cP^n}[S_i = x | \pi]\right) \\
&\le& \frac{1}{n} \sum_{i=1}^n \left( \sum_{x \in  G_l (\pi,\epsilon,\delta)} q(x) \cdot \frac{\Pr_{S \sim \cP^n}[\pi | S_i = x ] \cdot \Pr_{S \sim \cP^n}[S_i = x]}{\Pr[\pi]} + \sum_{x \notin G_l (\pi,\epsilon,\delta)} \Pr_{S \sim \cP^n}[S_i = x | \pi] \right)\\
&\leq& \frac{e^{\epsilon}}{1-\sqrt{\delta}} \cdot \frac{1}{n} \sum_{i=1}^n \left( \sum_{x \in  G_l (\pi,\epsilon,\delta)} q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x] + \Pr_{x \sim \cP_\pi} \left[ x \notin G_l (\pi,\epsilon,\delta) \right] \right)\\
&\le& \frac{e^{\epsilon}}{1-\sqrt{\delta}}  \cdot \frac{1}{n} \sum_{i=1}^n \left( \sum_{x \in \cX } q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x] + \delta^{1/4}  \right) \quad (w.p. \ 1 - \delta^{1/4} \text{ by Claim \ref{bpi} }) \\
&=& \frac{e^{\epsilon}}{1-\sqrt{\delta}} \, q(\cP) + \delta^{1/4} \quad (w.p. \ 1 - \delta^{1/4})
\end{eqnarray*}

Additionally:
\begin{align*}
q(Q_\pi) &= \frac{1}{n} \sum_{i=1}^n \left(\sum_{x \in G_u (\pi,\epsilon,\delta)} q(x) \cdot \Pr_{S \sim \cP^n}[S_i = x | \pi] + \sum_{x \notin G_u (\pi,\epsilon,\delta)} q(x) \cdot \Pr_{S \sim \cP^n}[S_i = x | \pi] \right) \\
&\ge  \frac{1}{n} \sum_{i=1}^n \sum_{x \in  G_u (\pi,\epsilon,\delta)} q(x) \cdot \frac{\Pr_{S \sim \cP^n}[\pi | S_i = x ] \cdot \Pr_{S \sim \cP^n}[S_i = x]}{\Pr[\pi]} \\
&\ge e^{-\epsilon}(1-\sqrt{\delta})  \cdot \frac{1}{n} \sum_{i=1}^n \sum_{x \in  G_u (\pi,\epsilon,\delta)} q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x] \\
&= e^{-\epsilon}(1-\sqrt{\delta}) \cdot \frac{1}{n} \sum_{i=1}^n \left(  \sum_{x \in \cX } q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x] - \sum_{x \notin G_u (\pi,\epsilon,\delta)} q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x]\right) \\
&\ge e^{-\epsilon}(1-\sqrt{\delta}) \cdot \frac{1}{n} \sum_{i=1}^n \left(  \sum_{x \in \cX } q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x] - \Pr_{x \sim \cP} \left[ x \notin G_u (\pi,\epsilon,\delta)\right]\right) \\
&\ge e^{-\epsilon}(1-\sqrt{\delta}) \cdot \frac{1}{n} \sum_{i=1}^n \left(  \sum_{x \in \cX } q(x) \cdot  \Pr_{S \sim \cP^n}[S_i = x] - \delta^{1/4} \right) \quad (w.p. \ 1 - \delta^{1/4} \text{ by Claim \ref{bpi} })\\
&= e^{-\epsilon}(1-\sqrt{\delta}) \left( q(\cP) - \delta^{1/4} \right) \quad (w.p. \ 1 - \delta^{1/4})
\end{align*}
Therefore, with probability at least $1-2\delta^{1/4}$ over the selection of $\pi$:
$$
| q(Q_\pi) - q(\cP) | \le \frac{e^{\epsilon}}{1-\sqrt{\delta}} - 1 + \delta^{1/4}
$$
\end{proof}


\begin{theorem}[Transfer Theorem for $(\epsilon,\delta)$-Pointwise Indistinguishability]
\label{thm:transfer2}
Suppose that $M$ is $(\epsilon,\delta)$-pointwise indistinguishable and $(\alpha,\beta)$-sample accurate. Then for every index $j$ indexing a linear query it also satisfies:
$$\Pr_{S \sim \cP^n, \pi \sim M(S)}[|a_j - \E_{S \sim \cP^n}[q_j(S)]| \geq \alpha +\sqrt{\beta}+ \frac{e^{\epsilon}}{1-\sqrt{\delta}} - 1 + \delta^{1/4}] \leq \sqrt{\beta} + 2\delta^{1/4}$$
i.e. it is $(\alpha', \beta')$-distributionally accurate for $\alpha' = \alpha +\sqrt{\beta}+\frac{e^{\epsilon}}{1-\sqrt{\delta}} - 1 + \delta^{1/4}$ and $\beta' = \sqrt{\beta} + 2\delta^{1/4}$.
\end{theorem}

Identically to the case of $(\epsilon,0)$-pointwise stability, we can use Lemma \ref{lem:monitor} to lift the distributional accuracy guarantees of Theorem \ref{thm:transfer2} to a guarantee of uniform distributional accuracy:

\begin{corollary}
\label{thm:uniform-transfer}
Suppose that $M$ is $(\epsilon,\delta)$-pointwise indistinguishable and $(\alpha,\beta)$-uniformly sample accurate. Then  it also satisfies:
$$\Pr_{S \sim \cP^n, \pi \sim M(S)}[\max_j|a_j - \E_{S \sim \cP^n}[q_j(S)]| \geq \alpha +\sqrt{\beta}+ \frac{e^{\epsilon}}{1-\sqrt{\delta}} - 1 + \delta^{1/4}] \leq \sqrt{\beta} + 2\delta^{1/4}$$
i.e. it is $(\alpha', \beta')$-uniformly distributionally accurate for $\alpha' = \alpha +\sqrt{\beta}+\frac{e^{\epsilon}}{1-\sqrt{\delta}} - 1 + \delta^{1/4}$ and $\beta' = \sqrt{\beta} + 2\delta^{1/4}$.
\end{corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\saeed{Trying to prove Transfer for $(\epsilon,\delta)$ case using the trick that gets better dependence on $\beta$.}
\begin{lemma}
\label{lem:tech2'}
Fix $x \in \cX$, $\boldx \in \cX^n$, and $i \in [n]$. If $M$ is $(\epsilon,\delta)$-pointwise indistinguishable:
\begin{itemize}
\item with probability $1-\delta^{2/3}$ over the draw of $\pi \sim \pirv | S_{<i} = \boldx_{<i}$:
$$\Pr[\pirv = \pi | S_{<i} = \boldx_{<i} ] \leq \frac{e^\epsilon}{1-\delta^{1/3}} \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}, S_i = x]$$
\item with probability $1-\delta^{2/3}$ over the draw of $\pi \sim \pirv| S_{<i} = \boldx_{<i}, S_i=x$:
$$ \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}, S_i = x] \leq \frac{e^\epsilon}{1-\delta^{1/3}} \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}]$$
\end{itemize}
\end{lemma}

\begin{proof}
In this proof, we will use the following definitions of bad and good sets of transcripts:
\begin{definition}
We define the \emph{bad and good} sets of transcripts $\pi$ given a pair of data points $x,x'$ and a dataset $\boldx_{-i} \in \cX^{n-1}$ at level $\epsilon \geq 0$ as:
$$G(\boldx_{-i},x,x',\epsilon) = \{\pi \in \pispace: e^{-\epsilon} \leq \frac{\Pr[\textrm{Interact}(M, A; \boldx_{-i},x) = \pi]}{\Pr[\textrm{Interact}(M, A; \boldx_{-i},x') = \pi]} \leq e^{\epsilon}\}$$
$$B(\boldx_{-i},x,x',\epsilon) = \pispace \setminus G(\boldx_{-i},x,x',\epsilon) =  \{\pi : \pi \not\in G(\boldx_{-i},x,x',\epsilon)\}$$
\end{definition}
Note that by the definition of $(\epsilon,\delta)$-pointwise indistinguishability, it is immediate that for any $\boldx_{-i}, x, x'$: $\Pr[\pirv \in B(\boldx_{-i},x,x',\epsilon) | S = (\boldx_{-i}, x')] \leq \delta$.

We prove each part of the lemma in turn. First, for any transcript $\pi$, we have:
\begin{align*}
&\Pr[\pirv = \pi | S_{<i} = \boldx_{<i} ] \\
&= \sum_{(x', \boldx'_{>i})}\Pr[S_{\ge i} = (x', \boldx'_{>i})] \Pr[\pirv = \pi | S = (\boldx_{<i},x',\boldx'_{>i})] \\
&= \sum_{(x', \boldx'_{>i}): \pi \in G(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{\ge i} = (x' ,\boldx'_{>i})] \Pr[\pirv = \pi | S = (\boldx_{<i},x',\boldx'_{>i})]\\
&+ \sum_{(x' , \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{\ge i} = (x' , \boldx'_{>i})] \Pr[\pirv = \pi | S = (\boldx_{<i},x',\boldx'_{>i})]  \\
&\leq \sum_{(x' , \boldx'_{>i}): \pi \in G(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{\ge i} = (x' , \boldx'_{>i})] \cdot e^{\epsilon} \Pr[\pirv = \pi | S = (\boldx_{<i},x,\boldx'_{>i})] \\
&+ \sum_{(x' , \boldx'_{>i}):\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{\ge i} = (x' , \boldx'_{>i})] \Pr[\pirv = \pi | S = (\boldx_{<i},x',\boldx'_{>i})]  \\
&\leq e^\epsilon \Pr[\pirv = \pi|S_{<i} = \boldx_{<i}, S_i = x] +  \sum_{(x' , \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{\ge i} = (x' , \boldx'_{>i})] \Pr[\pirv = \pi | S = (\boldx_{<i},x',\boldx'_{>i})] \\
&= e^\epsilon \Pr[\pirv = \pi|S_{<i} = \boldx_{<i}, S_i = x] + \sum_{(x' , \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)} \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] \Pr[S_{\ge i} = (x' , \boldx'_{>i})  | \pirv = \pi, S_{<i} = \boldx_{<i}] \\
&=e^\epsilon \Pr[\pirv = \pi|S_{<i} = \boldx_{<i}, S_i = x] + \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] \cdot \underbrace{\sum_{(x' , \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)} \Pr[S_{\ge i} = (x' , \boldx'_{>i})  | \pirv = \pi, S_{<i} = \boldx_{<i}]}_{:=g(\pi,\boldx_{<i})} \\
&= e^\epsilon \Pr[\pirv = \pi|S_{<i} = \boldx_{<i}, S_i = x] + \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] \cdot g(\pi,\boldx_{<i})
\end{align*}

Let's bound $g(\pi,\boldx_{<i})$ with high probability. We have that:
\begin{align*}
&\E_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ g(\pi,\boldx_{<i}) \right]  \\
&= \sum_{\pi} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}] \sum_{(x', \boldx'_{>i})}  \Pr[S_{\ge i} = (x' , \boldx'_{>i})  | \pirv = \pi, S_{<i} = \boldx_{<i}] \1 [\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)] \\
&= \sum_{\pi} \sum_{(x', \boldx'_{>i})} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}] \cdot \frac{\Pr [\pirv = \pi | S=(\boldx_{<i}, x', \boldx'_{>i})] \Pr [S_{\ge i} = (x' , \boldx'_{>i})]}{ \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}]} \1 [\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)] \\
&= \sum_{(x', \boldx'_{>i})} \Pr [S_{\ge i} = (x' , \boldx'_{>i})] \sum_{\pi} \Pr [\pirv = \pi | S=(\boldx_{<i}, x', \boldx'_{>i})] \1 [\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)] \\
&= \E_{(x', \boldx'_{>i}) \sim S_{\ge i}} \left[ \underbrace{\Pr_{\pi \sim \pirv} \left[ \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon) | S=(\boldx_{<i}, x', \boldx'_{>i}) \right]}_{\le \delta \quad \text{by $(\epsilon, \delta)$-pointwise indistinguishability}} \right] \\
&\le \delta
\end{align*}

Finally, by Markov's inequality,
$$
\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ g(\pi,\boldx_{<i}) > \delta^{1/3} \right] \le \delta^{2/3}
$$


In the reverse direction:
\begin{align*}
&\Pr[\pirv = \pi| S_{<i} = \boldx_{<i}, S_i = x] \\
&= \sum_{(x', \boldx'_{>i})}\Pr[S_{>i} = \boldx'_{>i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{<i},x, \boldx'_{>i})] \\
&=\sum_{(x', \boldx'_{>i}): \pi \in G(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)} \Pr[S_{>i} = \boldx'_{>i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{<i},x, \boldx'_{>i})] \\
&+\sum_{(x', \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)} \Pr[S_{>i} = \boldx'_{>i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{<i},x, \boldx'_{>i})] \\
&\leq \sum_{(x', \boldx'_{>i}): \pi \in G(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{>i} = \boldx'_{>i}]\cdot\Pr[S_i = x']\cdot e^\epsilon \Pr[\pirv = \pi| S = (\boldx_{<i},x', \boldx'_{>i})] \\
&+\sum_{(x', \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)} \Pr[S_{>i} = \boldx'_{>i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{<i},x, \boldx'_{>i})] \\
&\leq e^\epsilon \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] +  \sum_{(x', \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_{>i} =\boldx'_{>i}]\cdot\Pr[S_i = x']\cdot\Pr[\pirv = \pi| S = (\boldx_{<i},x, \boldx'_{>i})] \\
&=  e^\epsilon \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] \\
&+  \sum_{(x', \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)} \Pr[S_i = x']\cdot \Pr[S_{>i} = \boldx'_{>i}]\cdot \frac{\Pr[S_{>i} = \boldx'_{>i}| \pirv = \pi, S_{<i} = \boldx_{<i}, S_i=x]\cdot \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}, S_i = x]}{\Pr[S_{>i} = \boldx'_{>i}| S_{<i} = \boldx_{<i}, S_i = x]} \\
&= e^\epsilon \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] \\
&+ \Pr[\pirv = \pi| S_{<i} = \boldx_{<i}, S_i = x]\cdot \underbrace{\sum_{(x', \boldx'_{>i}): \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)}\Pr[S_i = x']\cdot \Pr[S_{>i} = \boldx'_{>i}| \pirv = \pi, S_{<i} = \boldx_{<i}, S_i=x]}_{:=g(\pi, x, \boldx_{<i})} \\
&= e^\epsilon \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}] + \Pr[\pirv = \pi| S_{<i} = \boldx_{<i}, S_i = x] \cdot g(\pi, x, \boldx_{<i})
\end{align*}

We have that
\begin{align*}
&\E_{\pi \sim \pirv | S_{<i} = \boldx_{<i}, S_i = x} \left[ g(\pi, x, \boldx_{<i}) \right]  \\
&= \sum_{\pi} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}, S_i =x] \sum_{(x', \boldx'_{>i})} \Pr[S_i = x']\cdot \Pr[S_{>i} = \boldx'_{>i}| \pirv = \pi, S_{<i} = \boldx_{<i}, S_i=x] \1 [\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)] \\
&= \sum_{\pi} \sum_{(x', \boldx'_{>i})} \Pr [\pirv = \pi| S_{<i} = \boldx_{<i},, S_i =x] \Pr[S_i = x'] \frac{\Pr[\pirv = \pi | S=(\boldx_{<i},x, \boldx'_{>i})] \Pr [S_{>i} = \boldx'_{>i}]}{\Pr [\pirv = \pi | S_{<i} = \boldx_{<i}, S_i = x] }  \1 [\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)] \\
%&=  \sum_{\pi} \sum_{(\boldx_{-i},x')} \Pr[S = (\boldx_{-i}, x')] \Pr[\pirv = \pi | S = (\boldx_{-i}, x)] \1 [\pi \in B(\boldx_{-i},x,x',\epsilon)]  \\
&=  \sum_{(x', \boldx'_{>i})} \Pr[S_{\ge i} = (x', \boldx'_{>i})] \sum_{\pi} \Pr[\pirv = \pi | S=(\boldx_{<i},x, \boldx'_{>i})] \1 [\pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon)] \\
&=  \E_{(x', \boldx'_{>i}) \sim S_{\ge i}} \left[ \underbrace{\Pr_{\pi \sim \pirv} \left[ \pi \in B(\boldx_{<i}, \boldx'_{>i},x,x',\epsilon) | S=(\boldx_{<i}, x, \boldx'_{>i}) \right]}_{\le \delta \quad \text{by $(\epsilon, \delta)$-pointwise indistinguishability}} \right] \\
&\le \delta
\end{align*}

Hence, by Markov's inequality,
$$
\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}, S_i = x} \left[ g(\pi, x, \boldx_{<i}) > \delta^{1/3} \right] \le \delta^{2/3}
$$
\end{proof}


\begin{lemma}\label{lem:epsdelta-posterior}
If $M$ is $(\epsilon,\delta)$-pointwise indistinguishable, then for any data distribution $\cP$, any $j$ indexing a linear query, and any $\eta \in (0,1)$:
$$\Pr_{(S,\pirv)} \left[|q_j(S)-q_j(\cP)| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \eta + 2n \delta^{1/3}$$
\end{lemma}

\begin{proof}
Triangle inequality implies:
\begin{align*}
&\Pr_{(S,\pirv)} \left[ \left| q_j(S)-q_j(\cP) \right| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&\le \Pr_{(S,\pirv)} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&+ \Pr_{(S,\pirv)} \left[ \left| \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3}\right] \\
&\le \Pr_{(S,\pirv)} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&+ \sum_{i=1}^n \Pr_{(S,\pirv)} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3}\right]
\end{align*}

Let's focus on each term separately. First, we have that
\begin{align*}
&\Pr_{(S,\pirv)} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&= \E_{\pi \sim \pirv} \left[ \underbrace{\Pr_{S \sim Q_\pi} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv = \pi,  S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right]}_{ \le \eta \quad \text{(by Azuma's inequality, just as in the warmup $(\epsilon,0)$ case)}} \right] \\
&\le \eta
\end{align*}

Now fix $i \in [n]$. We have that
\begin{align*}
& \Pr_{(S,\pirv)} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3}\right] \\
&=  \Pr_{(S_{<i},\pirv)} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3}\right] \\
&= \E_{\boldx_{<i} \sim S_{<i}} \left[ \Pr_{ \pi \sim (\pirv | S_{<i} = \boldx_{<i})} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv = \pi, S_{< i} = \boldx_{<i}]-q_j(\cP) \right| > \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3}\right] \right]
\end{align*}

So it suffices to show that for any $\boldx_{<i}$, with probability $1 - 2 \delta^{1/3}$ over the draw of $\pi \sim (\pirv | S_{<i} = \boldx_{<i})$,
$$
\left| \E_{S_i} [q_j (S_i) | \pirv=\pi, S_{< i} = \boldx_{<i}]-q_j(\cP) \right| \le \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3}
$$

Fix $\boldx_{<i}$. Given a transcript $\pi$ and $\boldx_{<i}$, define:
$$
G_u (\boldx_{<i}, \pi) = \left\{x \in \cX : \Pr[ \pirv = \pi | S_{<i} = \boldx_{<i} ] \leq \frac{e^\epsilon}{1-\delta^{1/3}} \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}, S_i = x] \right\}
$$
$$
G_l (\boldx_{<i}, \pi) = \left\{x \in \cX : \Pr[\pirv = \pi | S_{<i} = \boldx_{<i}, S_i = x] \leq \frac{e^\epsilon}{1-\delta^{1/3}} \Pr[ \pirv = \pi | S_{<i} = \boldx_{<i} ] \right\}
$$

\begin{claim}\label{bpi2}
We have that:
\begin{itemize}
\item With probability at least $1 - \delta^{1/3}$ over $\pi \sim (\pirv | S_{<i} = \boldx_{<i})$:
$$\Pr_{x \sim \cP}[x \notin G_u (\boldx_{<i}, \pi) ] \le \delta^{1/3}$$
\item With probability at least $1 - \delta^{1/3}$ over $\pi \sim (\pirv | S_{<i} = \boldx_{<i})$:
$$\Pr_{x \sim S_i | \pirv = \pi, S_{<i} = \boldx_{<i}}[x \notin G_l (\boldx_{<i}, \pi) ] \leq \delta^{1/3}$$
\end{itemize}
\end{claim}

\begin{proof}
Observe that Lemma \ref{lem:tech2'} and elementary probability imply:
$$
\E_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \Pr_{x \sim \cP}[x \notin G_u (\boldx_{<i}, \pi) ] \right] = \E_{x \sim \cP} \left[ \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}}[x \notin G_u (\boldx_{<i}, \pi)] \right] \le \delta^{2/3}
$$
$$
\E_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \Pr_{x \sim S_i | \pirv = \pi, S_{<i} = \boldx_{<i} }[x \notin G_l (\boldx_{<i}, \pi) ] \right] = \E_{x \sim S_i} \left[ \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}, S_i = x  }[x \notin G_l (\boldx_{<i}, \pi)] \right] \le \delta^{2/3}
$$
Markov's inequality completes the proof.
\end{proof}

We have that
\begin{align*}
&\E_{S_i} [q_j (S_i) | \pirv=\pi, S_{< i} = \boldx_{<i}] \\
&=  \sum_x q_j(x)\cdot \Pr [S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] \\
&= \sum_{x \in G_l (\boldx_{<i}, \pi) } q_j (x)\cdot \Pr [S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] + \sum_{x \notin G_l (\boldx_{<i}, \pi) } q_j(x)\cdot \Pr [S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] \\
&\le \sum_{x \in G_l (\boldx_{<i}, \pi) } q_j (x)\cdot \frac{\Pr [\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]\cdot \Pr [S_i = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } + \sum_{x \notin G_l (\boldx_{<i}, \pi) } \Pr [S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}]\\
&\leq  \frac{e^\epsilon}{1-\delta^{1/3}} \cdot \sum_x q_j(x)\cdot \Pr_{S \sim \cP^n}[S_i = x] + \Pr_{x \sim S_i | \pirv = \pi, S_{<i} = \boldx_{<i}} \left[ x \notin G_l (\boldx_{<i}, \pi) \right]\\
&\le \frac{e^\epsilon}{1-\delta^{1/3}} \cdot q_j (\cP) + \delta^{1/3} \quad (\text{w.p. $1 - \delta^{1/3}$ over $\pi \sim (\pirv | S_{<i} = \boldx_{<i})$ by Claim \ref{bpi2}} )
\end{align*}
Also,
\begin{align*}
&\E_{S_i} [q_j (S_i) | \pirv=\pi, S_{< i} = \boldx_{<i}] \\
&= \sum_x q_j (x)\cdot \Pr [S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] \\
&\ge \sum_{x \in G_u (\boldx_{<i}, \pi) } q_j (x)\cdot \Pr [S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] \\
&= \sum_{x \in G_u (\boldx_{<i}, \pi) } q_j (x)\cdot \frac{\Pr [\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]\cdot \Pr [S_i = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } \\
&\ge e^{-\epsilon} (1 - \delta^{1/3}) \cdot \sum_{x \in G_u (\boldx_{<i}, \pi) } q_j (x) \cdot \Pr [S_i = x] \\
&= e^{-\epsilon} (1 - \delta^{1/3}) \cdot \left( \sum_{x } q_j (x) \cdot \Pr [S_i = x] - \sum_{x \notin G_u (\boldx_{<i}, \pi) } q_j (x) \cdot \Pr [S_i = x] \right) \\
&\ge e^{-\epsilon} (1 - \delta^{1/3}) \cdot \left( q_j (\cP) - \Pr_{x \sim \cP} \left[ x \notin G_u (\boldx_{<i}, \pi) \right]\right) \\
&\ge e^{-\epsilon} (1 - \delta^{1/3}) \cdot \left( q_j (\cP) - \delta^{1/3} \right) \quad (\text{w.p. $1 - \delta^{1/3}$ over $\pi \sim (\pirv | S_{<i} = \boldx_{<i})$ by Claim \ref{bpi2} } )
\end{align*}
completing the proof.
\end{proof}



\begin{theorem}[Transfer Theorem for $(\epsilon,\delta)$-Pointwise Indistinguishability]
\label{thm:transfer2'}
Suppose that $M$ is $(\epsilon,\delta)$-pointwise indistinguishable and $(\alpha,\beta)$-sample accurate with respect to $f$. Then for every index $j$ indexing a linear query and any $\eta \in (0,1)$ it also satisfies:
$$\Pr_{S \sim \cP^n, \pirv \sim I(M, \cA, f; S)} \left[ \left|a_j - q_j(\cP) \right| \geq \alpha +\frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \leq \beta + \eta + 2n\delta^{1/3}$$
i.e. it is $(\alpha', \beta')$-distributionally accurate with respect to $f$ for $\alpha' = \alpha +\frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta + \eta + 2n\delta^{1/3}$.
\end{theorem}
\begin{proof}
Fix an index $j$. Triangle inequality implies:
\begin{align*}
& \Pr_{(S,\pirv)} \left[ \left|a_j - q_j(\cP) \right| \geq \alpha +\frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \\
&\le \Pr_{(S,\pirv)} \left[ \left|a_j - q_j(S) \right| \geq \alpha  \right] + \Pr_{(S,\pirv)} \left[ \left| q_j(S) - q_j(\cP) \right| \geq \frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \\
&\le \beta + \eta + 2n\delta^{1/3}
\end{align*}
where we used $(\alpha,\beta)$-sample accuracy and Lemma \ref{lem:epsdelta-posterior}.
\end{proof}

Identically to the case of $(\epsilon,0)$-pointwise stability, we can use Lemma \ref{lem:monitor} to lift the distributional accuracy guarantees of Theorem \ref{thm:transfer2'} to a guarantee of uniform distributional accuracy:

\begin{corollary}
\label{thm:uniform-transfer'}
Suppose that $M$ is $(\epsilon,\delta)$-pointwise indistinguishable and $(\alpha,\beta)$-uniformly sample accurate. Then for all $\eta \in (0,1)$ it also satisfies:
$$\Pr_{S \sim \cP^n, \pi \sim I(S)} \left[ \max_j \left|a_j - q_j(\cP) \right| \geq \alpha +\frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \leq \beta + \eta + 2n\delta^{1/3}$$
i.e. it is $(\alpha', \beta')$-uniformly distributionally accurate for $\alpha' = \alpha +\frac{e^{\epsilon}}{1-\delta^{1/3}} - 1 + \delta^{1/3} + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta + \eta + 2n\delta^{1/3}$.
\end{corollary}
\saeed{dependence on $\beta$ is improved but we lose a factor of $n$ in $2n\delta^{1/3}$ using the new argument.}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
\saeed{Trying an alternative proof for $(\epsilon,\delta)$-DP: Moshe's idea + Azuma:}
\begin{lemma}\label{lem:noidea}
Fix an index $i$ and $\boldx_{<i}$. If $M$ is $(\epsilon, \delta)$-DP, then we have that for any $j$ indexing a linear query:
$$
\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \left| \E_{S_i} \left[ q_j (S_i) | \pirv = \pi , S_{<i} = \boldx_{<i} \right]  - q_j (\cP) \right| > 3(e^\epsilon - 1) \right] \le \frac{\delta}{e^\epsilon -1}
$$
\end{lemma}
\begin{proof}
For simplicity, let's call $\E_{S_i} \left[ q_j (S_i) | \pirv = \pi , S_{<i} = \boldx_{<i} \right] := g_j (\pi, \boldx_{<i})$. Define for an $\alpha > 0$:
$$
\pispace_\alpha = \left\{ \pi \in \pispace | \, g_j (\pi, \boldx_{<i}) - q_j (\cP) > \alpha \right\}
$$
$$
\cX_{+} (\pi) = \left\{ x \in \cX | \, \Pr \left[ S_i = x | \pirv=\pi, S_{<i} = \boldx_{<i} \right] > \Pr \left[ S_i = x \right] \right\}
$$
$$
B_\alpha^+ = \bigcup_{\pi \in \pispace_\alpha} \left( \cX_{+} (\pi) \times \{ \pi \} \right)
$$
$$
\pispace_\alpha^+ (x) = \left\{ \pi \in \pispace | (x,\pi) \in B_\alpha^+ \right\}
$$
Let $\alpha = 3(e^\epsilon - 1)$. Suppose, towards a contradiction, that $\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \left| g_j (\pi, \boldx_{<i})  - q_j (\cP) \right| > \alpha \right] > \frac{\delta}{e^\epsilon -1}$. So we must have that $\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ g_j (\pi, \boldx_{<i})  - q_j (\cP) > \alpha \right] > \frac{\delta}{2(e^\epsilon -1)}$ or $\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ q_j (\cP) - g_j (\pi, \boldx_{<i})  > \alpha \right] > \frac{\delta}{2(e^\epsilon -1)}$. Without loss of generality, assume
\begin{equation}\label{eq:delta}
\Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ g_j (\pi, \boldx_{<i})  - q_j (\cP) > \alpha \right] = \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \pi \in \pispace_\alpha \right]> \frac{\delta}{2(e^\epsilon -1)}
\end{equation}
We have that
\begin{align*}
&\Pr_{(x,\pi) \sim (S_i, \pirv)|S_{<i} = \boldx_{<i}} \left[ (x,\pi) \in B_\alpha^+ \right] - \Pr_{x \sim S_i, \pi \sim  (\pirv | S_{<i} = \boldx_{<i}) } \left[ (x,\pi) \in B_\alpha^+ \right] \\
&= \sum_{\pi \in \pispace_\alpha} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}] \sum_{x \in \cX_{+} (\pi)} \left( \Pr [S_i = x | \pirv = \pi, S_{<i} = \boldx_{<i}] - \Pr [S_i = x] \right) \\
&\ge \sum_{\pi \in \pispace_\alpha} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}] \sum_{x \in \cX } q_j(x) \left( \Pr [S_i = x | \pirv = \pi, S_{<i} = \boldx_{<i}] - \Pr [S_i = x] \right) \\
&= \sum_{\pi \in \pispace_\alpha} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}] \left( g_j (\pi, \boldx_{<i}) - q_j (\cP) \right) \\
&> \alpha \cdot \sum_{\pi \in \pispace_\alpha} \Pr [\pirv = \pi | S_{<i} = \boldx_{<i}] \\
&= \alpha \cdot \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \pi \in \pispace_\alpha \right]
\end{align*}
On the other hand, using the guarantee of $(\epsilon, \delta)$-differential privacy:
\begin{align*}
&\Pr_{(x,\pi) \sim (S_i, \pirv)|S_{<i} = \boldx_{<i}} \left[ (x,\pi) \in B_\alpha^+ \right] - \Pr_{x \sim \cP, \pi \sim  (\pirv | S_{<i} = \boldx_{<i}) } \left[ (x,\pi) \in B_\alpha^+ \right] \\
&= \sum_{x \in \cX} \Pr [ S_i = x ] \left( \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i} , S_i =x} \left[\pi \in \pispace_\alpha^+ (x) \right] - \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[\pi \in \pispace_\alpha^+ (x) \right] \right) \\
&\le \sum_{x \in \cX} \Pr [ S_i = x ] \left( (e^\epsilon - 1) \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[\pi \in \pispace_\alpha^+ (x) \right] + \delta \right) \\
&= (e^\epsilon - 1) \Pr_{x \sim \cP, \pi \sim  (\pirv | S_{<i} = \boldx_{<i}) } \left[ (x,\pi) \in B_\alpha^+ \right] + \delta \\
&\le (e^\epsilon - 1) \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \pi \in \pispace_\alpha \right] + \delta \\
& < (e^\epsilon - 1) \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \pi \in \pispace_\alpha \right] + 2(e^\epsilon - 1) \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \pi \in \pispace_\alpha \right] \quad \text{(by Equation \ref{eq:delta})}\\
&= \alpha \cdot \Pr_{\pi \sim \pirv | S_{<i} = \boldx_{<i}} \left[ \pi \in \pispace_\alpha \right]
\end{align*}
a contradiction.
\end{proof}

\begin{lemma}\label{lem:epsdelta-posterior2}
If $M$ is $(\epsilon,\delta)$-DP, then for any data distribution $\cP$, any $j$ indexing a linear query, and any $\eta \in (0,1)$:
$$\Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[|q_j(S)-q_j(\cP)| >  3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \eta + \frac{n\delta}{e^\epsilon - 1}$$
\end{lemma}

\begin{proof}
Triangle inequality implies:
\begin{align*}
&\Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| q_j(S)-q_j(\cP) \right| >3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&\le \Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&+ \Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > 3(e^\epsilon -1) \right] \\
&\le \Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&+ \sum_{i=1}^n \Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > 3(e^\epsilon -1) \right]
\end{align*}

Let's focus on each term appearing in RHS separately. First, we have that
\begin{align*}
&\Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv, S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \\
&= \E_{\pi \sim \pirv} \left[ \underbrace{\Pr_{S \sim Q_\pi} \left[ \left| q_j(S)- \frac{1}{n} \sum_{i=1}^n  \E_{S_i} [q_j (S_i) | \pirv = \pi,  S_{< i}] \right| > \sqrt{\frac{2\ln(2/\eta)}{n}}\right]}_{ \le \eta \quad \text{(for all $\pi$'s by Azuma's inequality, just as in the warmup case)}} \right] \\
&\le \eta
\end{align*}

Now fix an index $i \in [n]$. We have that
\begin{align*}
& \Pr_{S \sim \cP^n,\pirv \sim I(S)} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > 3(e^\epsilon -1) \right] \\
&=  \Pr_{(S_{<i},\pirv)} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv, S_{< i}]-q_j(\cP) \right| > 3(e^\epsilon -1) \right] \\
&= \E_{\boldx_{<i} \sim S_{<i}} \left[ \underbrace{\Pr_{ \pi \sim (\pirv | S_{<i} = \boldx_{<i})} \left[ \left| \E_{S_i} [q_j (S_i) | \pirv = \pi, S_{< i} = \boldx_{<i}]-q_j(\cP) \right| > 3(e^\epsilon -1) \right]}_{\le \frac{\delta}{e^\epsilon - 1} \quad \text{(for all $\boldx_{<i}$ by Lemma \ref{lem:noidea})}} \right] \\
&\le \frac{\delta}{e^\epsilon - 1}
\end{align*}
completing the proof.
\end{proof}

\begin{theorem}[Transfer Theorem for $(\epsilon,\delta)$-Differential Privacy]
\label{thm:transfer2''}
Suppose that $M$ is $(\epsilon,\delta)$-DP and $(\alpha,\beta)$-sample accurate with respect to $f$. Then for every index $j$ indexing a linear query and any $\eta \in (0,1)$:
$$\Pr_{S \sim \cP^n, \pirv \sim I(M, \cA, f; S)} \left[ \left|a_j - q_j(\cP) \right| \geq \alpha +3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \leq \beta + \eta + \frac{n\delta}{e^\epsilon - 1}$$
i.e. $M$ is $(\alpha', \beta')$-distributionally accurate with respect to $f$ for $\alpha' = \alpha +3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta + \eta + \frac{n\delta}{e^\epsilon - 1}$.
\end{theorem}
\begin{proof}
Fix an index $j$. Triangle inequality implies:
\begin{align*}
& \Pr_{S \sim \cP^n,\pirv \sim I(M, \cA, f; S)} \left[ \left|a_j - q_j(\cP) \right| \geq \alpha + 3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \\
&\le \Pr_{S \sim \cP^n,\pirv \sim I(M, \cA, f; S)} \left[ \left|a_j - q_j(S) \right| \geq \alpha  \right] + \Pr_{S \sim \cP^n,\pirv \sim I(M, \cA, f; S)} \left[ \left| q_j(S) - q_j(\cP) \right| \geq 3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \\
&\le \beta + \eta + \frac{n\delta}{e^\epsilon - 1}
\end{align*}
where we used $(\alpha,\beta)$-sample accuracy and Lemma \ref{lem:epsdelta-posterior2}.
\end{proof}

Identically to the case of $(\epsilon,0)$-differential privacy, we can use Lemma \ref{lem:monitor} to lift the distributional accuracy guarantees of Theorem \ref{thm:transfer2''} to a guarantee of uniform distributional accuracy.

\begin{corollary}
\label{thm:uniform-transfer''}
Suppose that $M$ is $(\epsilon,\delta)$-DP and $(\alpha,\beta)$-uniformly sample accurate. Then for all $\eta \in (0,1)$ it also satisfies:
$$\Pr_{S \sim \cP^n, \pi \sim I(S)} \left[ \max_j \left|a_j - q_j(\cP) \right| \geq \alpha +3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}} \right] \leq \beta + \eta + \frac{n\delta}{e^\epsilon - 1}
$$
i.e. it is $(\alpha', \beta')$-uniformly distributionally accurate for $\alpha' = \alpha +3(e^\epsilon -1) + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta + \eta + \frac{n\delta}{e^\epsilon - 1}
$.
\end{corollary} 

==> uniform.tex <==
%!TEX root = main.tex
\subsection{Bounds for Uniform $(\epsilon, \delta)$-Indistinguishability and the Gaussian Mechanism}
\saeed{do we want the Gaussian Mech in the title here if it is going to be discussed under applications?}\ar{NOTE THIS SECTION IS DEFUNCT -- TURNS OUT UNIFORM INDISTINGUISHABILITY SAME AS $(\epsilon,0)$-DP...}
We now begin to generalize our argument from Section \ref{sec:warmup} to handle the case of $(\epsilon,\delta)$-pointwise indistinguishability. We'll complete this task in Section \ref{sec:delta}: the main difficulty to overcome will be that in the definition of pointwise indistinguishability (Definition \ref{def:pointwise}), the ``bad event'' which occurs with probability $\delta$ over $\pi \sim I(S)$: that $\left| \log \frac{\Pr[\pirv = \pi | S]}{\Pr[\pirv = \pi|S']} \right| > \epsilon$---is \emph{non-uniform}: i.e. it might be different for each neighboring pair $(S, S')$.

However, some very important algorithms---in particular, the Gaussian Mechanism---satisfy a stronger \emph{uniform} indistinguishability guarantee, which makes the proof of the transfer theorem as easy as it was in Section \ref{sec:warmup}. We introduce the notion here:


\begin{definition}
A mechanism $M$ satisfies $(\epsilon,\delta)$-uniform indistinguishability if for all data analysts $\cA$, datasets $S$, and post-processing functions $f:\pispace\rightarrow\pispace$, with probability $1-\delta$ over the draw of $\pi \sim \textrm{Interact}(M, A, f; S)$:
$$ \sup_{S \sim S'}\frac{\Pr[ \pirv = \pi | S]}{\Pr[ \pirv = \pi | S'] } \leq e^\epsilon$$
$$\inf_{S \sim S'}\frac{\Pr[ \pirv = \pi | S]}{\Pr[ \pirv = \pi | S'] } \geq e^{-\epsilon}$$
where $S \sim S'$ means $S,S'$ are neighboring data sets and that $\Pr[\cdot]$ operator denotes either a probability density or probability mass.
\end{definition}

The only thing we need to do to generalize the transfer theorem from Section \ref{sec:warmup} to $(\epsilon,\delta)$-uniform indistinguishability is to prove an analogue of Lemma \ref{lem:warmup-posterior}. We do so here: the modifications needed are minimal.
%We now reproduce an analogue of Lemma~{} for an $(\epsilon, \delta)$-uniformly indistinguishable algorithm.



\begin{lemma}\label{lem:uniform}
If $M$ is $(\epsilon,\delta)$-uniformly indistinguishable, then for any data distribution $\cP$ and any linear query $q$, if $S \sim \cP^n$, with probability $1-\delta$ over the draw of $\pi \sim \textrm{Interact}(M, A, f; S)$, for any $\eta \in (0,1)$:
$$\Pr_{S \sim Q_{\pi}}\left[|q(S)-q(\cP)| \geq (e^{\epsilon}-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \eta$$

\end{lemma}
\begin{proof}
Once again, similar to the proof of Lemma \ref{lem:warmup-posterior}, we can apply Azuma's inequality to conclude:
\begin{equation}
\label{eq:azuma2}
\Pr\left[\left|\frac{1}{n}\sum_{i=1}^n q(S_i) - \frac{1}{n} \sum_{i=1}^n  \E[q(S_i) | S_{< i}]\right|\geq t \right] \leq 2\exp\left(\frac{-t^2n}{2}\right)
\end{equation}
Now fix any realization $\boldx$, and consider each term: $\E[q(S_i) | S_{< i} = \boldx_{<i}]$. We again have:
\begin{eqnarray*}
\E_{S \sim Q_\pi}[q(S_i) | S_{< i} = \boldx_{<i}] &=&  \sum_x q(x)\cdot \Pr_{S \sim \cP^n}[S_i = x | \pirv=\pi, S_{<i} =\boldx_{< i}] \\
&=& \sum_x q(x)\cdot \frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{< i}, S_i = x]\cdot \Pr_{S \sim \cP^n}[S_i = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } \\
\end{eqnarray*}

Now consider the term $\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{< i}, S_i = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] }$ that we wish to bound by $e^\epsilon$. Recall that uniform indistinguishability guarantees us that with probability $1-\delta$ over the choice of $\pi$, $\sup_{S \sim S'} \frac{\Pr[\pirv = \pi | S]}{\Pr[\pirv = \pi | S']} \leq e^\epsilon$. Whenever this occurs, we have for any $i$:


\begin{eqnarray*}
\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } &=&
\frac{\sum_{\boldx'_{\geq i}}\Pr[\pirv = \pi | S = (\boldx_{<i}, x, \boldx_{> i}')]\Pr_{S \sim P^n}[S_{ \geq i} = \boldx'_{\geq i}]}{\sum_{\boldx'_{\geq i}}\Pr[\pirv = \pi |S = (\boldx_{<i}, \boldx'_{\geq i})]\Pr_{S \sim P^n}[S_{ \geq i}=\boldx'_{\geq i}]} \\
&\leq& \sup_{S \sim S'} \frac{\Pr[\pirv = \pi | S]}{\Pr[\pirv = \pi | S']} \\
&\leq& e^\epsilon
\end{eqnarray*}
%$$
% \leq \sup_{S_{< i}}\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{ > i}, S_i = x, S_{< i}]}{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{ > i}, S_{< i}]} \leq  \sup_{S_{< i}, x'}\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{ > i}, S_i = x, S_{< i}]}{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{ > i}, S_i = x', S_{< i}]}  \leq e^{\epsilon},
%$$

%
%\cj{Trying to be more careful each step.}
%\begin{align*}
%&\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{< i}, S_i = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] }\\
%&= \frac{\sum_{\boldx'_{> i}}\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_i = x, S_{ > i} =\boldx'_{>i}]\Pr_{S \sim P^n}[S_{ > i} = \boldx'_{>i}]}{\sum_{\boldx'_{> i}}\Pr[\pirv = \pi |S_{< i} =\boldx_{< i}, S_{> i } = \boldx'_{> i} ]\Pr_{S \sim P^n}[S_{ > i} = \boldx'_{> i}]}\\
%&\leq \sup_{\boldx'_{> i}}\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_i = x, S_{ > i} = \boldx'_{> i} ]}{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_{ > i}=\boldx'_{> i} ]} \\
%&= \sup_{\boldx'_{> i}}\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_i = x, S_{ > i} =\boldx'_{> i} ]}{\sum_{x'} \Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_i = x', S_{ > i} = \boldx'_{> i} ] \cdot \Pr[S_i = x']} \\
%&\le \sup_{\boldx'_{> i}, x'}\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_i = x, S_{ > i} =\boldx'_{> i} ]}{\Pr_{S \sim \cP^n}[\pirv = \pi | S_{< i} = \boldx_{<i}, S_i = x', S_{ > i} =\boldx'_{> i} ]} \\
%&\le \sup_{\boldx \sim \boldx'}\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S = \boldx]}{\Pr_{S \sim \cP^n}[\pirv = \pi | S = \boldx']} \\
%&\leq e^{\epsilon},
%\end{align*}
%\cj{Since $\boldx$ is already used, maybe we should do something different for the second to last line?}


The reverse inequality $\frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } \geq e^{-\epsilon}$ follows symmetrically. Hence with probability $1-\delta$ over $\pi \sim I(S)$, simultaneously for all $i$:
$$e^{-\epsilon}q(\cP) \leq \E_{S \sim Q_\pi}[q(S_i) | S_{< i}] \leq e^\epsilon q(\cP)$$
%\begin{eqnarray*}
%\E_{S \sim Q_\pi}[q(S_i) | S_{< i}] &=& \sum_x q(x)\cdot \frac{\Pr_{S \sim \cP^n}[\pirv = \pi | S_i = x, S_{< i} = \boldx_{< i}]\cdot \Pr_{S \sim \cP^n}[S_j = x]}{\Pr[\pirv = \pi | S_{< i} =\boldx_{< i}] } \\
%&\leq&  \sum_x q(x)\cdot \Pr_{S \sim \cP^n}[S_j = x] = e^{\epsilon}q(\cP), \text{ and symmetrically:} \\
%\E_{S \sim Q_\pi}[q(S_i) | S_{< i}] &\geq& e^{-\epsilon}q(\cP) \\
%\end{eqnarray*}
%Hence with probability $1-\delta$ over the draw of $\pi$:
% $$e^{-\epsilon}q(\cP) \leq \frac{1}{n} \sum_{i=1}^n  \E[q(S_i) | S_{< i}]\leq e^\epsilon q(\cP).$$
 Combining this with Equation \ref{eq:azuma2} gives us that for any $\eta > 0$, with probability $1-\eta-\delta$ \saeed{this $1-\eta-\delta$ probability is with respect to the joint of $(\pi,S)$, so we better say for all good $\pi$'s, with probability $1-\eta$ when $S \sim Q_{\pi}$ ...} when $S \sim Q_{\pi}$:
 $$q(S) \leq e^\epsilon q(\cP) + \sqrt{\frac{2\ln(2/\eta)}{n}} \ \ \textrm{and} \ \ q(S) \geq e^{-\epsilon} q(\cP) - \sqrt{\frac{2\ln(2/\eta)}{n}}$$
 \end{proof}

 With Lemma \ref{lem:uniform} in hand, we can again combine it with the Bayesian Resampling Lemma (Lemma \ref{lem:resamp}) as we did in Section \ref{sec:warmup} to obtain a transfer theorem for $(\epsilon,\delta)$-uniform indistinguishability: The proof is identical to the proof of Lemma \ref{thm:main-warmup} except that we use Lemma \ref{lem:uniform} in place of Lemma \ref{lem:warmup-posterior}.

 \begin{theorem}\label{thm:gauss_transfer}
 Suppose that $M$ is $(\epsilon, \delta)$-uniformly pointwise indistinguishable and $(\alpha, \beta)$-sample accurate with respect to $f$. Then for every $j$ indexing a linear query, and any $\eta \in (0,1)$ it also satisfies:
 $$\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A,f;S)}\left[|a_j - q_j(\cP)| \geq \alpha +(e^\epsilon-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \beta + \eta + \delta$$
i.e. it is $(\alpha', \beta')$-distributionally accurate with respect to $f$ for $\alpha' =  \alpha +(e^\epsilon-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta +\eta + \delta$.
 \end{theorem}

Similarly, we can apply Lemma \ref{lem:monitor} to obtain a uniform accuracy bound:
\begin{corollary}
 Suppose that $M$ is $(\epsilon, \delta)$-uniformly pointwise indistinguishable and $(\alpha, \beta)$-uniformly sample accurate with respect to $f$. Then for any $\eta \in (0,1)$ it also satisfies:
 $$\Pr_{S \sim \cP^n, \, \pirv \sim \textrm{Interact}\,(M,A,f;S)}\left[\max_j|a_j - q_j(\cP)| \geq \alpha +(e^\epsilon-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}\right] \leq \beta + \eta + \delta$$
i.e. it is $(\alpha', \beta')$-uniformly distributionally accurate for $\alpha' =  \alpha +(e^\epsilon-1) + \sqrt{\frac{2\ln(2/\eta)}{n}}$ and $\beta' = \beta +\eta + \delta$.
\end{corollary}


